A Universal Question-Answering Platform for Knowledge Graphs

Knowledge from diverse application domains is organized as knowledge graphs (KGs) that are stored in RDF engines accessible in the web via SPARQL endpoints. Expressing a well-formed SPARQL query requires information about the graph structure and the exact URIs of its components, which is impractical for the average user. Question answering (QA) systems assist by translating natural language questions to SPARQL. Existing QA systems are typically based on application-specific human-curated rules, or require prior information, expensive pre-processing and model adaptation for each targeted KG. Therefore, they are hard to generalize to a broad set of applications and KGs. In this paper, we propose KGQAn, a universal QA system that does not need to be tailored to each target KG. Instead of curated rules, KGQAn introduces a novel formalization of question understanding as a text generation problem to convert a question into an intermediate abstract representation via a neural sequence-to-sequence model. We also develop a just-in-time linker that maps at query time the abstract representation to a SPARQL query for a specific KG, using only the publicly accessible APIs and the existing indices of the RDF store, without requiring any pre-processing. Our experiments with several real KGs demonstrate that KGQAn is easily deployed and outperforms by a large margin the state-of-the-art in terms of quality of answers and processing time, especially for arbitrary KGs, unseen during the training.

==> algorithms/filtering_algorithm.tex <==
\begin{algorithm}[t]
\caption{Filtration Algorithm}\label{alg:filtration}
\hspace{1em} \textbf{Input:} $q_{result}$: result of executing SPARQL query and \{$answer_{dtype}$, $answer_{type}$\} \\
\hspace{1em} \textbf{Output:} Filtered answer list $ans_{list}$.
\hline
\begin{algorithmic}[1]
\State $ans_{list} \gets []$
\For{answer in $q_{result}$}
    \State $datatype \gets ExtractAnsDataTypeFromQuery(answer)$
    \If{datatype = $answer_{dtype}$}
        \If{datatype in \{Numeric, Date, Boolean\}}
            \State $ ans_{list}.append(answer) $
        \Else 
            \State $answerType \gets ExtractTypeFromQuery(answer) $
            \State $score \gets  $ 
                semanticSimilarity($answer_{type}$, answerType)
            \If{score > 0.5}
                \State $ ans_{list}.append(answer) $
            \EndIf
        \EndIf
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

==> algorithms/linking_algorithm.tex <==
\begin{algorithm}[t]
\caption{Just-in-time linking algorithm}
\label{alg:linking}
% \hspace{1em} 
\textbf{Input:} PGP from Question Understanding \\
% \hspace{1em} 
\textbf{Output:} PGP annotated with vertices and predicates from  KG %\hline
\begin{algorithmic}[1]
\For{node in N}
    \State $query \gets createVertexSparqlQuery(node.label)$
    \State $candidateVertices \gets executeSparql(query)$
    \State $candidateScores \gets $
    semanticSimilarity(node.label, candidateVertices )
    \State $assignTopKVerticesToNode(CandidateScores, k)$
\EndFor
\For{edge in E}
    \State $connectedNode \gets getConnectedNode(edge.label)$
    \State $query \gets createPredicateSparqlQuery(connectedNode)$
    \State $candidatePredicates \gets executeSparql(query)$
    \State $candidateScores \gets $ 
    semanticSimilarity(edge.label, candidatePredicates )
    \State $assignTopKPredicatesToEdge(candidatePredicates, k)$
\EndFor
\end{algorithmic}
\end{algorithm}

==> algorithms/training_model.tex <==
\begin{algorithm}[t]
\caption{Training question understanding model}
\label{alg:training}
\begin{flushleft}
\textbf{Input:} Training data($D$): \{$d$: (a question $q$, Set of triple patterns $TP$)\}, pre-trained language model $LM$, Number of epoch $N_E$, Batch size $B_{size}$, loss function $L$ \\
\textbf{Output:} Fine-tuned language model to perform the inference $trained\_model$
\end{flushleft}
\hline
\begin{algorithmic}[1]
\State $current\_model \gets Initialize(LM) $
\State $processed\_ts \gets \{\} $
\For{$(q, TP)$ in $D$}
    \State $y \gets F(TP)$
    
    \State $processed\_ts \gets processed\_ts.append(q, y)$
\EndFor
\For{$i$ in $N_E$}
    \State $ B \gets Divide(processed\_ts, B_{size})$
    \For{$j$ in range($B$)}
        \State $loss = L(current\_model, B_j)$
        \State $current\_model \gets update\_model(current\_model, loss)$
    \EndFor
\EndFor
\State $trained\_model \gets current\_model$
\end{algorithmic}
\end{algorithm}

==> algorithms/triples_extraction.tex <==
\begin{algorithm}[t]
\caption{Triples Extraction Model Training}\label{alg:triples}
\hspace{1em} \textbf{Input:} input natural language question (q) \\
\hspace{1em} \textbf{Output:} List of Triples (T)
\hline
\begin{algorithmic}[1]
\State $num\_encoders, num\_decoders \gets 12 $
\State $ques\_emb \gets Embedding(q)$
\State $enc\_layer\_input \gets ques\_emb$
\While{ i < num\_encoders}
\State $ques\_self \gets SelfAttention(enc\_layer\_input)$
\State $self\_norm \gets Norm(ques\_self + enc\_layer\_input)$
\State $feed\_forward \gets FeedForward(self\_norm)$
\State $encoder\_output \gets Norm(feed\_forward + self\_norm)$
\State $enc\_layer\_input \gets encoder\_output$
\EndWhile
% \State $ encoder\_vector \gets enc\_layer\_input$
% \State $triples\_seq \gets preprocess(T)$
% \State $triples\_emb \gets Embedding(triples\_seq)$
% \State $dec\_layer\_input \gets triples\_emb$
\State $dec\_layer\_input \gets prepareDecoderInput(enc\_layer\_input)$
\While{ i < num\_decoders}
\State $triples\_self \gets SelfAttention(dec\_layer\_input)$
\State $self\_norm \gets Norm(triples\_self + dec\_layer\_input)$
\State $cross\_att \gets CrossAttention(self\_norm, encoder\_vector)$
\State $cross\_norm \gets Norm(cross\_att + self\_norm)$
\State $feed\_forward \gets FeedForward(cross\_norm)$
\State $decoder\_output \gets Norm(feed\_forward + cross\_norm)$
\State $dec\_layer\_input \gets decoder\_output$
\EndWhile
% \State $ decoder\_vector \gets dec\_layer\_input$
% \State $probabilities \gets Softmax(decoder\_vector)$
% \State $output \gets max(probabilities)$
% \State $triples \gets postprocess(output)$
\State $triples \gets prepareOutput(dec\_layer\_input)$
\State \Return triples
\end{algorithmic}
\end{algorithm}

==> sections/ack.tex <==
\section{Acknowledgement}
\label{sec:ack}

We would like to thank the authors of EDGQA, gAnswer, and Falcon for responding to our questions and providing the necessary information to reproduce their results. 

% Also, we would like to thank the Falcon’s authors for responding to our questions and providing the necessary information to index DBpedia, Yago, DBLP and MAG.

==> sections/comparative_analysis_submitted.tex <==
\section{Background and Limitations}
\label{sec:comp}

This section provides the necessary background of SPARQL-based QA systems and techniques adopted by these systems, as summarized in Table~\ref{tab:background}. These systems commonly follow two main steps: \myNum{i} \emph{question understanding} (\emph{QU}) to extract the key entities and relations from the given question and generate an intermediate abstract representation, and \myNum{ii} \emph{linking} this abstract representation to corresponding KG's vertices and predicates to construct basic graph patterns (\emph{BGPs}), i.e., the building blocks of a SPARQL query. 
Some QA systems, such as EDGQA, include a step for \emph{filtering} the potential answers that could be retrieved by the \emph{BGPs}. For the \emph{filtering} step, existing systems build prior knowledge of all node types in a KG during the pre-processing phase. The \emph{filtering} is done by \emph{linking} the detected unknown in the abstract representation to KG's types and extending the generated \emph{BGPs} with an extra triple pattern, e.g., \RDFTYPE{?sea}{a}{dbo:Sea}. Finally, the systems send the final SPARQL queries to the RDF engine for execution, i.e., the received answers are \emph{pre-filtered}. This section highlights the \emph{QU} and \emph{linking} techniques adopted by the top-performing systems: gAnswer~\cite{gAnswer2014, gAnswer2018}, EDGQA~\cite{EDGQA}, and  NSQA~\cite{NSQA}. These systems adopt different techniques that require a cumbersome process to work for a specific KG.\shorten 

\input{tables/comparison}

\subsection{Question Understanding}

The SPARQL-based QA systems utilize rule-based or deep learning-based mechanisms. EDGQA based on human-curated rules managed to outperform NSQA’s deep learning-based model in understanding questions and achieved better F1 scores in {\lcq}~\cite{lcquad} and {\qald}~\cite{qald9} benchmarks. Figure ~\ref{fig:understanding} shows the two main steps of understanding  $q^E$, which is a conjunctive question with an unknown entity connected to another two mentioned entities, \textbf{Danish Straits} and \textbf{Kaliningrad}, via two different relations, \textbf{flows} and \textbf{city on the shore}.  It is a challenging task to identify the unknown entity and its connections to the mentioned entities. As discussed below, both gAnswer and EDGQA failed to understand $q^E$.\shorten 

gAnswer converts the question to a semantic query graph (SQG) constructed from the entities and relations, which are extracted based on the syntactic dependency tree of the question and heuristic linguistic rules. In gAnswer, the Stanford dependency parser is used to map a question into a syntactic dependency tree. gAnswer adopts a node-first approach to extract entities or classes from a question, and then all question words starting with "WH" are extracted to represent an unknown entity. In SQG, forming triples is based on the dependency parse tree and heuristic rules.
Furthermore, gAnswer depends on a given set of relation mentions (synonyms); the source of this set in not mentioned in~\cite{gAnswer2018, gAnswer2014} but the files are provided in gAnswer’s repository\footnote{\url{https://drive.google.com/file/d/1hmqaftrTo0_qQNRApCuxFXaBx7SosNVy/view}}. Thus, gAnswer’s SQG may include relations that are not explicitly mentioned in the question. 
gAnswer's linguistic rules are curated based on the set of training questions in {\qald}. 
The final SQG generated by gAnswer for $q^E$ consists of the following triples: 
\RDFTYPE{city}{city of}{shore}, 
\RDFTYPE{city}{have name}{sea},
\RDFTYPE{sea}{which flow into}{Danish Straits},
\RDFTYPE{sea}{ have name}{Kalinigrad},
\RDFTYPE{sea}{have name}{shore}, 
\RDFTYPE{Kalinigrad}{shore}{shore}, and 
\RDFTYPE{Kalinigrad}{city of}{city}. gAnswer failed to detect the unknown entity and introduced relation phrases not in $q^E$, such as \emph{have name} and \emph{city of}. Hence, gAnswer generated unnecessary triples. Due to the irrelevant predicted triples,  gAnswer consumes more time in processing questions in {\lcq} than {\qald}, and achieves less F1 score.\shorten

EDGQA constructs an entity description graph (EDG) that represents a question. An EDG is a rooted acyclic graph and is divided into several blocks. Each block serves as a description of an entity. The EDG is created as follows: \myNum{i} the question is passed to  Stanford core NLP parser~\footnote{\url{https://stanfordnlp.github.io/CoreNLP/}} that constructs the constituency parsing tree of the question, and \myNum{ii} the resulting tree is used to create the final EDG by iteratively decomposing the question until no additional entity or description nodes are added. This iterative decomposition is a rule-based process.
%to detect the predefined phrase structure patterns from the tree and then decompose the descriptions into several sub-descriptions. 
The EDGQA’s rules were created based on questions in both {\lcq}~\cite{lcquad} and {\qald}~\cite{qald9}, which helped EDGQA outperform gAnswer and NSQA in both benchmarks. The EDGQA log of {\lcq}~\footnote{\url{https://github.com/HXX97/EDGQA/raw/main/query\_logs/query\_log\_test\_lc-quad\_2021\_07\_08\%2023\_48.txt}} include the generated SPARQL query for  $q^E$, where the generated EDG includes only one triple pattern: \RDFTYPE{unknown}{Danish Straits}{flow}. Surprisingly, EDGQA did not understand the full conjunctive question and missed the triple related to Kaliningrad. Moreover, EDGQA detected \emph{Danish Straits} as a relation and \emph{flow} as an entity.  We analyzed different questions and their corresponding trees. We find that EDGQA failed to understand questions whose trees are unbalanced.  

%Error propagation: Error in the tree will propagate to the 
%It is very costly to human annotated tree banks, which very costly 

\begin{figure}
\ncp\ncp
  \centering
  \includegraphics[width=0.97\columnwidth]{figures/expectedQU.pdf}
  \ncp\ncp\ncp\ncp\ncp\ncp\ncp
\caption{A system’s understanding of $q^E$ (a) detects \emph{Danish Straits} and \emph{Kaliningrad} as  mentioned entities and  \emph{sea} as an unknown entity, plus two relations \emph{flows} and \emph{city on the shore}, then (b) form them as two triple patterns. 
}
\label{fig:understanding}
\ncp\ncp\ncp
\end{figure}

NSQA uses deep learning to develop Abstract Meaning Representation (AMR) parser. NSQA is based on a neuro-symbolic framework called Logical Neural Network (LNN)~\cite{LNN} developed by IBM, which is not available for us to reproduce results of NSQA. We highlight AMR’s limitations based on the information provided in~\cite{NSQA}. This parsing technique converts the question into the AMR representation; a directed rooted acyclic graph of a question. AMR is trained based on relations gathered from Propbank, verb-oriented relations. Thus, it is unclear whether AMR can detect relations based only on noun phrases, such as \emph{city on the shore}. The highest recall reported by NSQA using AMR is less than EDGQA in both benchmarks. This indicates that EDGQA's rules-based model outperformed NSQA’s semantic parser. Moreover, the training of AMR demands a set of curated trees for different questions. 
The AMR accuracy is based on the diversity of these tress, i.e., covering different types of connections between entities and dealing with balance and unbalance trees. Unlike AMR, {\sysName} uses only a set of questions and their corresponding sequences of triples, i.e., entity, relation, entity, to train the model to directly detect entities/relations and form them as triples. Finally, AMR has different granularity than SPARQL. Thus, NSQA’s question understanding model has to be adjusted to work with new domains; see the discussion section in~\cite{NSQA}.

\subsection{Entity and Relation Linking}

\input{tables/expectedLinking}

In QA systems, the linking phase is to map entities and relations extracted from a question to vertices and predicates in a KG. Table~\ref{tab:expectedLinking} shows the expected output of this step for $q^E$. The target is to link the entity phrases \textbf{Danish Straits} and \textbf{Kaliningrad} to URIs of the corresponding vertices, and relation phrases \textbf{flows} and \textbf{city on the shore} to URIs of the corresponding predicate in the KG. Entity and relation linking are a challenging task for QA systems~\cite{LinLXLC20}. The QA systems are classified based on the adopted linking methods into index-based, such as gAnswer~\cite{gAnswer2014, gAnswer2018} and EDGQA~\cite{EDGQA}, or DL-based systems, such as NSQA~\cite{NSQA}. These linking methods are KG-specific and require a sophisticated pre-processing phase, which demands adjustment per KG, huge computing resources, and processing time. Moreover, KGs are frequently updated. 
For example, Wikipedia is updated at a rate of over 1.8 edits per second\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:Statistics}} which will result in hundreds of thousands of edits per day in the corresponding DBpedia KG, which is updated monthly\footnote{\url{https://www.dbpedia.org/resources/latest-core/}}. The Microsoft Academic Graph is updated every 1-2 
weeks~\footnote{\url{https://docs.microsoft.com/en-us/academic-services/graph/resources-faq}}.
These linking methods do not support incremental indexing or continuous learning. Thus, these factors hinder the adoption of QA systems in practice and obstruct the use of these systems as an on-demand service to immediately process a question against an arbitrary KG.

gAnswer developed an index-based linking method, which constructs two index dictionaries for entities and relations. The complexity of this process is polynomial to the number of vertices in the KG~\cite{gAnswer2018, gAnswer2014}.
The entity dictionary is the crossWikis dictionary~\cite{gAnswerDict} constructed from a Google Crawler of the web. Each entity in the dictionary is mapped to a corresponding vertex in the KG with a confidence score. For relation linking, gAnswer constructs a relation mention dictionary that maps relation mentions to their corresponding predicates. For example, the mention \emph{starred by} and its predicate \emph{starring} will have an entry in the index. However, gAnswer did not provide a method to extract relation mentions and their corresponding entity pairs. Instead, it indicated that this information could be generated based on NLP~\cite{PATTY} or n-gram~\cite{FaderSE11} methods. Moreover, gAnswer did not provide an approach for incrementally updating the two index dictionaries to deal with vertices or predicates removed or added to the KG.

EDGQA utilizes three indexing systems, namely Falcon~\cite{falcon}, EARL~\cite{earl}, and Dexter \cite{dexter}, to index a KG’s vertices and predicates. For linking, EDGQA \myNum{i} ensembles the results of the three systems to select the corresponding vertices, then \myNum{ii} uses them to limit the search space for relation linking by adopting the method proposed at~\cite{eearl}, finally, \myNum{iii} utilizes a BERT-based~\cite{bert} model to rank the list of vertices and predicates. 
These linking methods, such as Falcon~\cite{falcon}, index a given KG by extracting vertices and predicates with their associated description in the KG. 
For example, Falcon uses the predicates \emph{\url{http://www.w3.org/2000/01/rdf-schema\#label}} and  
\emph{\url{http://www.w3.org/2004/02/skos/core\#altLabel}} to collect more descriptions and synonyms for each vertex or predicate. Falcon performs Part-of-speech (POS) tagging and n-gram methods on these descriptions and generates tagged documents to store them in Elasticsearch. In Falcon, the entity and relation linking is enabled based on the powerful keyword search in Elasticsearch. For an arbitrary KG, the user should decide which predicates will be used to collect the deceptions of vertices and predicates. For example, vertices and predicates in the Microsoft Academic Graph are not connected to a \emph{label} predicate. Instead, a user will need to use different predicates, e.g., an author’s name to index vertices of type author and a paper’s title to index vertices of type paper. In these indexing methods, the pre-processing is proportional to the number of triples in the KG. 

NSQA divides the entity linking step into two parts. The first part is training a model to perform entity detection from the question, a BERT-based neural model is trained for entity detection using 3,651 questions from {\lcq} with manually annotated mentions along with Blink \cite{blink} for entity disambiguation, which takes as the input the entity mention and the list of candidates from the KG. NSQA has to encode the mentions and KG's vertices in the same vector space where the nearest candidates to the given entity mention are retrieved and ranked. For relation linking, NSQA uses SemRel~\cite{nsqa_linking} which takes a question and its AMR graph. In SemRel, a transformer-based neural model is trained to predict the relation. The model returns a list of candidate relations from the set of relations in the KG and ranks them. In NSQA, building the vector space, i.e., generating embedding for a KG's vertices and predicate, dominates the cost of the pre-processing phase. Moreover, the linking methods used by NSQA do not support continuous learning to adjust the pre-trained model based on the changes in the KG instead of working from scratch. 

\nsstitle{Discussion: Formalization and Consequences.}
Existing linking methods formalized the entity and relation (ER) linking problem as  \myNum{i} a keyword search on a database of tagged documents, such as Falcon~\cite{falcon} that indexes vertices and predicates of a KG as documents in Elasticsearch,  \myNum{ii} a lookup in an inverted index, such as gAnswer that constructs an inverted index to map synonyms to relevant vertices or predicates in a KG, and \myNum{iii} a transformation problem based on deep learning, which includes the maintenance of a vector space of the target KG. We aim to formalize the ER problem in a way that does not need a pre-processing phase, as discussed in Section~\ref{sec:linking}.  

==> sections/execution_manager_old.tex <==
\section{The {\sysName} Post-Filtering}
\label{sec:exec}

The {\sysName} post-filtering method percolates answers collected by executing the semantically equivalent queries; the role of filtering shifts from RDF engines to {\sysName}. Existing QASs, such as EDGQA, adopt a pre-filtering method that demands prior knowledge of all node types in a KG. {\sysName}, as an on-demand service, avoids this limitation by predicting the answer type of the unknowns, e.g., string, number, or date, and retrieve the node type of the variables in the generated SPARQL query. {\sysName} filters answers, whose type does not match the predicted one.      
As shown in Figure ~\ref{fig:Task3}, the input to this module is the annotated PGP (A) and the output are the answers to the question that will be returned to the user ans. The first step is traversing the Annotated PGP (A) and creating candidate basic graph patterns (BGPs) from it. For each $e_i \in A$, we create a triple per each URI in $P_i$. Then, we get all possible combinations between the triples corresponding to different edges in (A).\shorten  

\begin{definition}[Basic Graph Pattern (BGP)]
A Basic Graph Pattern is a set of  triple patterns \{$t_i$ such that i $\geq$ 1 \}. Each triple pattern $t_i$  is in the form <subject> <predicate> <object>.
\end{definition}

These BGPs are ranked depending on the similarity scores of the vertices and edges from the knowledge graph with the entities and relations from the questions. Each one of the candidate BGPs will be assigned a score by following equation ~\ref{bgp_score} where T is the set of triples of the BGP, |T| is the number of triples in the BGP, $s_{vt}$ = S(v, $n_{li}$) is the semantic similarity score between the vertex ($v \in V_i$) used in the triple (t) and the label of the node in the PGP $n_{li}$ and $s_{pt}$ is the semantic similarity score between the predicate ($p \in P_i$) used in the triple (t) and the label of the edge in the PGP.
\begin{equation}
    score = \frac{1}{2 |T|} \Sigma_{t \in {T}} (s_{vt} + s_{pt})
    \label{bgp_score}
\end{equation}

% Example of the generated BGPs for the running example is as mentioned in Figure ~\ref{fig:Task3} 


Then the highest ranked BGPs are converted to their corresponding SPARQL queries. The query executor sends these queries to be executed to a remote endpoint of the graph we want to query, and a list of answers is returned $q_{result}$. Finally, the retrieved list of answers $q_{result}$ is sent to the filtration module to decide which subset of the returned answers should be sent back to the user as the final answer to the input natural language question, (ans) = $Filtering(q_{result})$ such that (ans) $\subset q_{result}$. This filtration module operates with the help of the semantic similarity module explained in Section 5.1 and an answer type prediction module.

\begin{figure}
 \ncp\ncp
  \centering
  \includegraphics[width=\columnwidth]{figures/execution&Filteration.pdf}
  \ncp\ncp\ncp\ncp\ncp\ncp
\caption{The execution and Filtration phase uses the predicted answer type $t_p$, the annotated PGP, and the maximum number of equivalent SPARQL queries (K). {\sysName} generates a set of BGPs, and ranks them to create up to K queries. {\sysName} adjusts these queries with an optional triple pattern to return the type of the main unknown to match it with $t_p$ and filter wrong answers. }
\label{fig:filter}
\ncp\ncp
\end{figure}

\nsstitle{Filtration Module.} 
The last step of the {\sysName} pipeline is applying a filtration step on the answers returned from the SPARQL endpoint $q_{result}$. The input for this module are the results returned from the SPARQL endpoint $q_{result}$ and the pair of  ($answer_{dtype}$, $answer_{type}$) retrieved using the answer type prediction module, and the output is the filtered set of answers to the given question (ans).
The process is divided into two steps: filtering based on the answer data type, followed by filtering based on the answer type if the answer data type was a string.
For the first part we check the datatype for all the answers returned, this answer data type is already returned with the answer, and if they are the same datatype as $answer_{dtype}$ then the answer will be included, if the data types of the answer and $answer_{dtype}$ don't match then the answer is discarded. If the $answer_{dtype}$ is string, then we move to step two, otherwise the filtration process ends here.

For the string filtration, we use $answer_{type}$ along with the semantic similarity module. We extract the type of the answer from the knowledge graph by adding an Optional triple to extract the type while retrieving the result of the SPARQL query. An example of the updated query is in Figure ~\ref{fig:Task3} then we calculate the semantic similarity between the type of the answer extracted from the graph and the predicted answer type $answer_{type}$, if they are similar then this answer is added to the final list of answers otherwise it is discarded.\shorten

Finally, the filtered answers (ans) are returned to the user as our answers to the natural language question. Filtering out the unneeded outputs brought a good impact by improving the overall performance of {\sysName}. It significantly improved the precision of the system, which led to the increase in the F1 score. After the completion of phase 3, the output received for the given running example is as follows:
<http://dbpedia.org/resource/Baltic\_Sea>





==> sections/mapping_pgp_bgp.tex <==
\section{{\sysName} Just-in-Time Linking Approach}
\label{sec:linking}

In this section, we explain the second step of our pipeline, where we perform the linking task through mapping the nodes and edges to vertices and predicates from the KG, respectively.
We use a Just-in-Time linking approach presented in Algorithm 1. The Just-in-time approach increases the efficiency of the linking step and decreases the storage required, as it  doesn't require any index creation or pre-processing steps to be performed on the graph before starting the linking process. Eliminating the pre-processing steps allows {\sysName} to easily work with different knowledge graphs, as no prior work is needed before dealing with the new KG.  The input is the PGP constructed in the question understanding phase, and the output is an annotated PGP where each node from the PGP is updated with a list of vertices from the graph and each edge from the PGP is updated with a list of predicates from the targeted KG.

We use SPARQL queries to retrieve the required information from the knowledge graph on demand  based on the information extracted from the natural language question. These queries return the subset of the graph that is more probable to contain the required answer. As shown in Figure ~\ref{fig:architecture}, this step is divided into two sequential parts: Linking nodes, followed by linking edges using the fetched vertices. We will first explain the semantic similarity module used within the linking algorithm, then we will explain the details of the linking approach. 

% \begin{definition}[Annotated PGP]
% An annotated Phrase Graph Pattern is a PGP that contains KG related information.
% Where  each $n_i \in N$ is updated with a list of vertices $V_i$ from the KG matching the label of $n_i$. Each $e_i \in E$ is updated with a list of predicates $P_i$ from the KG matching the label of $e_i$
% \end{definition}

\subsection{Semantic Similarity Module}
This module calculates the similarity between two inputs labels using word and character level embeddings. It is used in multiple places in the linking approach. The word and character level embeddings convert the input labels into vectors. Then these vectors are used to get the similarity score using the technique introduced in \cite{similarity}.
For the word embeddings, we use glove model \cite{glove}. Glove is an unsupervised learning algorithm used to obtain vector representations for words.
The word level embeddings have the disadvantage of not being able to deal with unknown words, words that do not appear in their vocabulary dictionary. For these unknown words, word embedding techniques such as Glove usually produce the same vector for any unknown word, no matter how different they are from each other. Character level embeddings are used to solve this problem. we use Chars2Vec \footnote{\url{https://github.com/IntuitionEngineeringTeam/chars2vec}} as our character level embedding. Chars2Vec is implemented in a way that the similarity of word spellings is captured by the distance metric between the embeddings. For example, the word \textbf{Tirana} was unknown to Glove, so this was handled by Char2Vec.

After obtaining the vectors of all words in the two input labels either by using the word embeddings or the character level embeddings, equation \ref{eq:similarity} is used to calculate the final similarity $S(X, Y)$ between the two inputs $X, Y$ \cite{similarity}. Each vector is associated by a type attribute indicating whether it was calculated from the word embeddings or the character level embeddings. sim($x_i$, $y_j$) is the cosine similarity between the two vectors $x_i \in X $ and $y_j \in Y$ with the condition that both vectors are of the same type. If they are not from the same type, then the similarity is zero. In this equation, we calculate the pairwise similarity between all words of the two inputs, then we calculate the mean of this similarity as the final similarity between the two inputs.  

\begin{equation}
    S(X, Y) = \frac{\Sigma_{x_i \in X, y_j \in Y} sim(x_i, y_j)}{|X+Y|}
    \label{eq:similarity}
\end{equation}



\subsection{Linking Based on Semantic Search}

Algorithm 1 is a pseudocode of the {\sysName} entity and relation linking approach based on semantic search to annotate the PGP.

\nsstitle{Entity Linking.} The first part is to annotate the nodes $n_i \in N$ with $V_i$ a list of vertices from the target knowledge graph using the label of the node $n_{li} = \{w_h\}$ such that (h $\geq$ 1 and 1 $\leq$ i $\leq$ h)  . This label consists of one or more words $w_h$. The first step to annotate the nodes $n_i$ is to create a SPARQL query that retrieves the candidate vertices, as shown in line 2. We join the different words of $n_{li}$ to create a conjunctive query that represents the pattern to search for within the graph, for example if  $n_{li}$ is "Danish Straits" then the pattern is "Danish AND Straits". Then, we use the ask\_query in Figure~\ref{fig:v1} to check the existence of the $<$label$>$ predicate in the knowledge graph. If the label exists then we use the select\_with\_label query from Figure~\ref{fig:v1}  otherwise we use the select\_no\_label query from Figure~\ref{fig:v1}. 

The existence check performed by the ASK query is critical when dealing with knowledge graphs which do not contain the $<$label$>$ predicate, as using the select query only may lead to missing the possible vertices in case the graph we are dealing with contains the information we need, but it is not associated to the node using the $<$label$>$ predicate. It also makes it easier to deal with multiple different knowledge graphs. 
% Another approach would be executing the first select query with the label and if it returns no answer then execute the second select query which doesn't use the $<$label$>$ predicate, But we found this approach to be less efficient than the ask approach because running two select queries is generally less efficient than running a select and an ask query. 
On line 3, we execute the constructed query. The query searches the knowledge graph for vertices whose label contains the label of the node in the PGP. The result of executing this query is a list of candidate vertices $v_{candidates}$. The next step shown on line 4 is to rank the returned list to select the vertices that are most similar to the label. In order to do that, we use the semantic similarity module to assign a score for each of the retrieved vertices based on the similarity between the label of the node $n_{li}$ in the PGP and the label of the vertex in the knowledge graph, as shown in equation~\ref{eq:similarity}. 



The similarity module is used to further filter the results returned from the vertex retrieving query as, although, the returned result are all guaranteed to contain the pattern we are searching for, but it does not guarantee that the label is similar to the pattern for example, if we have the $n_{li}$ is Kaliningrad, and the results after executing the query were the two vertices: "Kaliningrad" and "Mayor of Kaliningrad", although the two vertices contains the word "Kaliningrad", we should only consider the first vertex because the second vertex is different, although its label contains the pattern. On line 5, the vertices are sorted according to this score and the top K vertices $V_i \subset v_{candidates}$ are chosen and assigned to the node.
For the running example, the top matching vertices to the entity "Danish Straits" are {\url{http://dbpedia.org/resource/Danish_Straits} and \url{http://dbpedia.org/resource/Danish_straits}}. The top matching vertices for the entity "Kaliningrad" are {\url{http://dbpedia.org/resource/Kaliningrad} and \url{http://dbpedia.org/resource/Yantar,_Kaliningrad}}

\input{algorithms/linking_algorithm}


\begin{figure}[t]
% \ncp\ncp
\small
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8}]
L = {$w_i$}; label of the node consisting of list of words
pattern = conjunctive query of L
rdf:label ; predicate that associates vertices in 
the knowledge graph to their label

\textbf{Label Existence query:} (ask\_query)
Prefix rdf: <http://www.w3.org/2000/01/rdf-schema#>
ASK { ?p rdf:label ?o }

\textbf{Vertex retrieval query with label:}(select\_with\_label)
Prefix rdf: <http://www.w3.org/2000/01/rdf-schema#>
Select distinct ?uri  ?label
Where {
?uri rdf:label ?label .
?label  <bif:contains> pattern . } 
Limit 400

\textbf{Vertex retrieval query without label:}(select\_no\_label)
Select distinct ?uri  ?label
Where {
?uri ?p ?label .
?label  <bif:contains> pattern . }
Limit 400
\end{Verbatim}
% \ncp\ncp\ncp\ncp
\caption{All Queries templates used to create the SPARQL query executed to get the candidate vertices matching a node }
\label{fig:v1}
% \ncp\ncp\ncp\ncp
\end{figure}



\nsstitle{Relation Linking.} The algorithm starts at line 7 to annotate the edges of the PGP given the labels of these edges and the vertices assigned to the nodes of the KG. The labels of the edges are used to match predicates from the graph and the assigned vertices are used to prune the search space, as instead of searching the whole graph we only consider the subset of the graph containing the chosen vertices, this makes the relation linking process more efficient because we will be sure that our chosen predicates are connected to the chosen vertices. For each edge, we start by specifying the nodes connected by this edge as shown on line 7. On line 8, we use the list of vertices $V_i$ assigned to each node to create two SPARQL queries: the first query aims to retrieving all predicates connected to this vertex as a subject ($Q\xrightarrow{?p_r}*$) and the second query aims to  retrieving all predicates connected to this vertex as an object ($*\xrightarrow{?p_l}Q$), where * represents anything, $?p_r$ is the set of predicated connected to vertex Q as subject, $p_l$ is the set of predicated connected to vertex Q as an object and $Q \in V_i$. 

The need for the two queries is due to the fact that the PGP is an undirected graph so can not know whether the predicate is connected to the vertex as a subject or an object without trying the two cases. An example of the two SPARQL queries for the edges connected to the first vertex in the running example are shown in Figure~\ref{fig:p1}. On line 9, the two queries are executed and their results are merged into one list $p_{candidates} = p_l \cup p_r$. On line 10, the semantic similarity module is used to assign each predicate in this list a score which reflects the similarity between the label of the edge in the PGP and the predicate, as shown in equation~\ref{eq:similarity}. The candidate predicates are sorted according to this similarity scores. Finally on line 11, the top $k$ predicates $P_i$ are assigned to the edge. For the running example ($q^E$), the top matching predicates for the relation "city on shore" are {\url{http://dbpedia.org/property/nearestCity} and \url{http://dbpedia.org/property/cities}}. The top matching predicate for the relation "flows" is {\url{http://dbpedia.org/property/outflow}}.
The final annotated PGP of $q^E$ is  shown in the Figure~\ref{fig:architecture}.


\begin{figure}[t]
\small
\begin{verbatim}
1 SELECT distinct ?p WHERE {
    <http://dbpedia.org/resource/Danish_Straits> ?p ?o .
  }  LIMIT 100
2 SELECT distinct ?p WHERE {
    ?s ?p <http://dbpedia.org/resource/Danish_Straits> .
  } LIMIT 100.
\end{verbatim}
% \ncp\ncp\ncp\ncp
\caption{The two SPARQL queries to find predicates connected to the chosen vertex. The first query with the vertex as \textit{Subject} and the second query with the vertex as \textit{Object}}
\label{fig:p1}
% \ncp\ncp\ncp\ncp
\end{figure}




==> sections/old-files/comparative_analysis_old.tex <==
\section{Background and Limitations}
\label{sec:comp}

\input{tables/comparison}

====

\hl{Paragraph moved here from the intro, in case you want to reuse some of the material}
A QAS maps a question into semantically equivalent SPARQL queries. In QASs, processing a question goes through two main steps: (i) \emph{question understanding} to extract \emph{phrase triple patterns}, which connect the identified unknown to the extracted entities and relationships as phrases in the question, and (ii) \emph{linking} these triple patterns to corresponding synonymous \texttt{subject}/\texttt{objects} or \texttt{predicate} to construct \emph{BGPs}. The  \emph{phrase triple patterns} is a cornerstone of the \emph{BGPs} to be eventually generated, while the predicted synonyms dominate the answers' correctness. Due to the high variability of KGs' domains, \emph{question understanding} should adjust dramatically for each domain to deal with various kinds of entities/relationships connected in different ways, e.g., a paper identified by a long title or a location known by a single name. Furthermore, RDF engines lack the support for built-in mechanisms to lookup \texttt{subject}/\texttt{objects} or \texttt{predicate} based on synonyms or semantic search. For example, RDF engines cannot identify that the predicate \emph{nearestCity} is a synonym for "city on shore". 

======


This section provides the necessary background for the process of Knowledge Graph Question Answering (KGQA). The target of the KGQA process is to take the input natural language question, convert it to its corresponding SPARQL query, then execute this query to get the answer. For proper execution of this process, the recent work moved towards dividing this process into small tasks, where these small tasks form a pipeline that ends with answering the question.

The steps of this pipeline are: 

\begin{enumerate}
    \item \underline{Question Understanding:} Understanding the question text through extracting the key entities and relations from the given question; the output of this step is a structure representing the question.     
    
    \item \underline{Linking}: Linking the entities and relations from the question understanding step to vertices and predicates from the knowledge graph that we are dealing with. 
    
    \item \underline{Execution and Filtration}: Creating the SPARQL query given the KG information obtained from the previous step and executing it. The execution can be followed by an optional filtration step that some systems don't perform. The optional filtering step filters the answers returned from the SPARQL endpoint before sending them back to the user to remove irrelevant answers. 
    \end{enumerate}
We will further explain the details of each step using the following top-performing systems:  NSQA \cite{NSQA}, EDGQA\cite{EDGQA}, gAnswer \cite{gAnswer2018} and QAMP \cite{QAMP}. Each of the systems presented has a different approach and as a consequence associated cost for each phase.

\subsection{Question Understanding}

The target of this step is to extract all the relevant information and keywords from the given natural language questions. Most systems use different semantic parsing techniques. Figure ~\ref{fig:understanding} explains the expected output from this step on the running example. The input is the natural language question and the output is divided into two parts. First, we need to extract the entities from the question, then the second step retrieves the relation phrases from the question and checks how they connect the entities to the unknown that we want to retrieve. For our example the entities are: \textbf{Danish Straits} and \textbf{Kaliningrad} and the relation phrases are \textbf{flows} and \textbf{city on the shore}. The unknown that we are asking about is connected to the entity \textbf{Danish Straits} using \textbf{flows} relation phrase, and it is also connected to entity \textbf{Kaliningrad} using \textbf{city on the shore} relation phrase.


EDGQA constructs an Entity Description graph (EDG) that represents the question. An EDG is a rooted acyclic graph with different node types (e.g. root and entity) and different types of relations connecting these nodes. It is divided into several blocks, where each block serves as a description of an entity and the relations connect these blocks. For creating the EDG: first, the question is passed to  Stanford core NLP parser \footnote{https://stanfordnlp.github.io/CoreNLP/} that constructs the constituency parsing tree of the question. The resulting tree is used to identify the question type. Then the resulting tree is again used to create the final EDG by iteratively decomposing the question until no additional entity or description nodes are added. 
This iterative decomposition process is rule-based, where the rules detect the predefined phrase structure patterns from the tree and then decompose the descriptions into several sub descriptions. The output of EDGQA on the running example~\footnote{\url{https://github.com/HXX97/EDGQA/raw/main/query\_logs/query\_log\_test\_lc-quad\_2021\_07\_08\%2023\_48.txt}(Question 147)} is \RDFTYPE{unknown}{Danish Straits}{flow} where it failed to understand the second part of the question relating the unknown to Kaliningrad.

gAnswer converts the question to a semantic query graph constructed from the semantic relations which are extracted from the question using the Stanford dependency parser. The relation extraction is based on the syntactic dependency tree of the question and heuristic linguistic rules. gAnswer also provides a node-first approach, where the first step extracts entities or classes from the question, and then all question words starting from "WH" are extracted to represent variable nodes. For adding edges between these nodes to create the semantic query graph, a heuristic based on the dependency parse tree of the question is used. For the running example, gAnswer managed to extract the correct entities, but in addition to them, three extra wrong entities were detected. This is due to the process followed to add new nodes to the semantic query graph. The process is starting with identifying a target node in dependency parse tree. The target is either the WH word or the first node if it is not a WH question. Starting from this target node, we move through the neighbors of it, when a node is a Noun or a question word starting with WH then a new node is added to the semantic query graph. This affects the performance of the system, as it eliminates the possibility to have a noun relation phrase similar to the city on shore phrase of the example. The relations of the semantic query graph are extracted from a file that contains a list of relation mentions. This file needs to created in pre-processing phase and as mentioned in \cite{gAnswer2014}, this file is assumed to be given as an input to the system. The DBpedia version of this file is provided in the paraphrase directory \footnote{\url{https://drive.google.com/file/d/1hmqaftrTo0_qQNRApCuxFXaBx7SosNVy/view}}


\begin{figure}
% \ncp\ncp
  \centering
  \includegraphics[width=\columnwidth]{figures/expectedQU.pdf}
%   \ncp\ncp\ncp\ncp\ncp\ncp\ncp\ncp\ncp\ncp
\caption{Steps for Question Answering, where the input and expected output from the question understanding step with a) extracted entities from the question and  b) extracted relation phrase and their connection to the entities and the variable}
\label{fig:understanding}
% \ncp\ncp\ncp
\end{figure}

NSQA uses Abstract meaning Representation (AMR) parsing. This technique of parsing converts the question into an AMR parse, which is a directed rooted acyclic graph representing the question. Nodes represent concepts and edges represent the relations between these concepts. These concepts and relations are gathered from different sources such as Propbank which is a verb-oriented resource, so it is hard to understand questions with noun relation phrases. The parser used is a stack-Transformer transition-based model \cite{NaseemSWFRB19}. For the example, it is expected that NSQA will not be able to extract the noun phrase "city on shore" as it is trained on PropBank.

QAMP performs two steps, where the first step identifies the question type using a BiLSTM model. In the second step, QAMP parses the question into a set of sequences, each sequence consisting of a set of entity, property and class references. This parsing task is modeled as a multi-class classification task. The input question is represented as a sequence of tokens. These sequence of tokens are used to train a sequence to sequence model that assigns labels to the different question tokens. These labels indicate if the question word is an entity, relation or a class. The model used is a biLSTM + CRF  neural network. It assigns one of the six supported labels to the tokens of the question. The entities and relations predicted are connected together to form a graph with the help of KG information (With the help of the output of the linking task).  Although {\sysName} uses a Seq2Seq model for question understanding, but our model is different as we use the Seq2Seq model for a text generation task and the encoder and decoder consists of transformers as opposed to the Bi-LSTMs used in QAMP.
Since they are training a model to do the understanding part, it is expected that they can extract up to two entities and relations

Linking aligns the information extracted from the question to the knowledge graph.
It is divided into two parts: Entity and Relation Linking. Entity linking means mapping the entities extracted from the question to vertices in the knowledge graph.
Relation Linking means mapping the relation phrases extracted from the question to predicates from the knowledge graph.
Some systems train entity detection models, others use off the shelf techniques to do the entity and relation linking.

Figure ~\ref{fig:linking} shows the expected output of this step on the running example. The target of the first part is to link the entities \textbf{Danish Straits} and \textbf{Kaliningrad} as shown in Figure ~\ref{fig:linking}(a) to their corresponding vertices from the knowledge graph, as shown in Figure ~\ref{fig:linking}(b). The target of the second part is to link the relation phrases \textbf{flows} and \textbf{city on the shore} to their corresponding predicates from the knowledge graph. This step is knowledge graph dependent, because the output vertices and predicates will change with changing the knowledge graph we are querying. In this example, we are using Dbpedia as our target KG.

EDGQA performs the linking step for each block in the EDG generated from the question understanding phase. Then the detected components are ranked and combined to generate candidate queries. For entity linking, an ensemble of three pre-existing tools, Dexter \cite{dexter}, EARL \cite{earl} and Falcon \cite{falcon} is used, and their output vertices are merged. These systems index the target knowledge graphs to map between the entities in the knowledge graph and their labels. Then the extracted set of vertices are ranked based on their semantic similarity with the entity using a BERT-based \cite{bert} semantic matching model.
For relation linking, EDGQA uses Ref. \cite{eearl} which extracts the predicate candidates given the entities. They use the hypothesis that relations in the questions are properties of the entities or properties of the types of these entities.
The output of EDGQA on the running example is $Danish\_Straits \rightarrow $ \url{http://dbpedia.org/resource/Danish\_straits}, $flow \rightarrow$ \url{http://dbpedia.org/ontology/outflow}.

gAnswer performs a pre-processing step before linking to construct two index dictionaries for entities and relations. The entity dictionary is the crossWikis dictionary that is constructed from a Google Crawler of the web \cite{gAnswerDict}. Each entity in the dictionary is mapped to a referring entity from the knowledge graph with a confidence score. The relation dictionary is constructed in a way that for each relation, there exists a list of pairs of entities that are connected using this relation in the knowledge graph.

\subsection{Linking}
\begin{figure}
% \ncp\ncp
  \centering
  \includegraphics[width=\columnwidth]{figures/expectedLinking.pdf}
%   \ncp\ncp\ncp\ncp
\caption{Linking step for Question Answering with a) linking extracted entities and extracted relation phrases to b) vertices and predicates from the KG respectively}
\label{fig:linking}
% \ncp\ncp\ncp
\end{figure}

NSQA divides the entity linking step into two parts. The first part is training a model to perform entity detection from the question, a BERT-based neural model is trained for entity detection using 3,651 questions from LCQuAD with manually annotated mentions along with Blink \cite{blink} for entity disambiguation, which takes as the input the entity mention and the list of candidates from the knowledge graph. It encodes all the inputs in the same vector space where the nearest candidates to the given entity mention are retrieved and ranked. On the other hand, KGQAn performs the entity linking by first executing a SPARQL query to get candidate vertices and then uses a Glove based semantic similarity model to rank these vertices. This way, KGQAn does not need to annotate the questions with the vertices (mentions) from the knowledge graph to train the model.
For relation linking, NSQA uses SemRel \cite{nsqa_linking} which takes as inputs: the question text, its AMR graph and the entities in the question marked and linked. In SemRel a transformer based neural model is trained for predicting the relation. The model returns a list of candidate relations from the set of relations in the KG and ranks them. KGQAn doesn't need to train a model to predict the relations from the knowledge graph, it relies on the results retrieved from querying the knowledge graph along with the semantic similarity module.
For entity linking, The list of vertices in training and testing parts of the KG have no common values
All the vertices from the knowledge graph are passed through a bert-based encoder and encoded to a vector space, for each entity, It is encoded to the same vector space as the vertices, then they run a nearst neigbor to get the closet candidates, and then they use another encoder to rank the nearest vertices.
The target of the training is to get the weights of the two encoders, but all vertices (in either training or testing) are encoded in the vector space
For relation linking The linked vertices is used as an input to this module beside the AMR and the question. the input question and target predicates are embedded in the same vector space
They use 2 encoders one for all target predicates and the other for the question and linearized AMR
They make experiments on two different KGs, they used the golden SPARQL query provided in the datasets to extract the relations. For Dbpedia they trained on LC-QuAD 1.0 and QALD-9. For Wikidata: we train out system on the LC-QuAD 2.0 train dataset

In QAMP, the labels of all entities and predicates from the target knowledge graph are indexed into two separate catalogs and embedded into two separate vector spaces using English FastText model \cite{fasttext}.
For entity linking, QAMP retrieves a ranked list of entities from the entity catalog that are most similar to the entity mention in the question, along with a confidence score representing the similarity between the entity from the question and the entity from the graph. The confidence score is calculated using BM25 function \cite{bm25}. The same process happens for relation linking, except for using the Magnitude library \cite{magnitudeLib} for calculating the confidence score using nearest neighbors in the fastText embedding space
The labels of all entities and predicates in the KG into two separate catalogs and embedded into two separate vector spaces, so it is expected to do well in linking as the index contains all predicates and vertices from the graph.


For the triples extraction task within the knowledge graph question answering systems, The existing systems rely on different models for entity and relation linking. Although they used different models such as machine learning models or Seq2Seq deep learning models for each of the entity and relation linking tasks, they didn't achieve a good performance. Unlike other systems, KGQAn uses a Seq2Seq model to extract triples. To the best of our knowledge, the only other attempt to use a Seq2Seq model within the QA system is the relation linking approach in \cite{ibmlinking}


\subsection{Execution and Filtration}
This step is an optional step at the end of the KBQA pipeline. In general, the approach used by the systems is  adding types constraints to the SPARQL query generated before sending it to the SPARQL endpoint. NSQA and gAnswer do not perform this step, but they return all answers from the SPARQL endpoint to the user.
EDGQA performs filtration primarily through types, where it uses the DBpedia Ontology as a type bank. It saves all existing types from DBpedia in one list. While parsing the question in the question understanding step, nouns which are not entities are marked with a type description. For example, the type of the unknown in our running example is \textbf{sea}. In the filtering step, the similarity between this noun and all types in the DBpedia ontology is calculated. The DBpedia type of the highest score is used as a constraint to limit the domain of the unknown.

QAMP filtering step is similar to EDGQA as it depends on types (classes of answers). In the question understanding step, one of the labels that are linked to the question words were classes. In their linking step, they match these classes with their corresponding classes from the knowledge graph using a HDT self index of the RDF graph. After the list of candidate answers is retrieved, only those that belong to the identified class from the knowledge graph are considered and sent back to the user.
QAMP filtration according to their paper: Finally, we also have an option to filter answers by considering only those entities in the answer set A that have one of the classes in C 

\subsection{Limitations}
For question understanding, existing systems rely on parser-based techniques as a first step to understand the question, then post-process the output of the parser to create the final understanding. This need an intensive manual work to create the rules that process the output of the parser. Moreover, some systems struggle with long questions because the rules are not well-designed to handle the output of the parser in such cases. 
For linking, all explained systems rely on building an index, explicitly or implicitly. Explicitly when creating the index is a prerequisite step to using the system. Implicitly, when the systems use tools that works with the help of a pre-built index. This slow down the ability of systems to work on new knowledge graphs because this requires building a new index for the graph or updating the used tools.
Another limitation related to the filtration module is the prerequisite to get all possible types that appear in the KG in a pre-processing step. This also increase the difficulty of dealing with different KGs. 

==> sections/old-files/introduction-essam1.tex <==
\section{Introduction}
 \label{sec:intro}
\sloppy
There is a steep rise in the popularity of knowledge graphs (KGs) across various industry sectors, such as life science, drugs, electric vehicle, finance, and e-commerce, as KGs enable novel AI applications for automating and improving the performance of several tasks. RDF engines are widely utilized to store KGs due to (i) the RDF model's simplicity for representing KG's entities and relationships as \RDFTYPE{subject}{predicate}{object}, where a relationship (\texttt{predicate}) and an entity (\texttt{subject} or \texttt{object}) are  identified via web-accessible URIs~\cite{AliSYHN22}, 
(ii) available extensions supporting inferencing and reasoning to automate intelligence and enrich KGs with new facts~\cite{BursztynGMR15,AMIE13}, and (iii) a powerful query language and request protocol (SPARQL), where remote users or applications can retrieve information from the KG via SPARQL queries~\cite{lusail}. Hence, there is a rapid growth in the number of KGs accessible via SPARQL endpoints. Forming these queries require prior knowledge about SPARQL, the schema of the KG, as well as the exact URIs of the entities and predicates. For most users, a question-answering system (QAS) is a more effective and convenient method to explore a KG easily using a natural language. QAS maps a user's question into semantically equivalent SPARQL queries. %However, QASs are not available by default for KGs. 
Thus, an on-demand QAS, as illustrated in Figure~\ref{fig:ondemandQAS}, is needed to enable many users to benefit from the available KGs. 

\begin{figure}
\ncp\ncp
  \centering
  \includegraphics[width=.77\columnwidth]{figures/ondemandQAS.pdf}
  \ncp\ncp\ncp\ncp\ncp\ncp\ncp\ncp
\caption{Due to the rapid growth in the number of KGs accessible via SPARQL endpoints lacking natural language support, there is a need for an on-demand question-answering system (QAS) to process a user's question immediately against an arbitrary KG.}
\label{fig:ondemandQAS}
\ncp\ncp\ncp\ncp\ncp\ncp\ncp\ncp
\end{figure}

These KGs cover a vast set of domains, such as scientific publications, encyclopedias, bioinformatics, and politics.
Examples of these KGs for scientific publications are (i) Microsoft Academic Graph~\footnote{\url{https://makg.org/}} that contains eight billion triples about scientific publications, authors, and institutions, (ii) DBLP \footnote{https://dblp.org/}, which includes the information about major computer science journals and proceedings, and (iii) OpenCitations \footnote{\url{https://opencitations.net/sparql}} that provides bibliographic citation information. Consider for encyclopedias KGs (i) DBpedia~\footnote{\url{https://dbpedia.org/sparql}}, which is one of the largest general linked open data gathered from different Wikimedia projects, (ii) Wikidata~\footnote{\url{https://query.wikidata.org/}}, which is also a structured data of several Wikimedia projects, (iii) YAGO~\footnote{\url{https://yago-knowledge.org/sparql}} that combines information from Wikidata and schema.org%, which is the standard ontology of classes and relations
. Examples of KGs for bioinformatics and politics are Bio2RDF~\footnote{\url{https://bio2rdf.org/sparql}} and the UK Parliament~\footnote{\url{https://api.parliament.uk/sparql}}, respectively. 
  
A user expresses a question regarding KG's entities and relationships using synonyms. As an example, question $UQ$ in Figure~\ref{fig:nlq} finds \emph{the name of the sea into which Danish Straits flows and has Kaliningrad as one of the city on the shore}. A QAS has to extract the entities and relationships, identify the unknown, and finally link an entity or relationship to synonymous \texttt{subject}/\texttt{objects} or \texttt{predicate} in the target KG, respectively. Then, the QAS constructs a SPARQL query similar to that in Figure~\ref{fig:nlq}. In QASs, processing a user’s question goes through two main steps: (i) \emph{question understanding} to capture and extract \emph{triple patterns} mainly connecting the identified unknown to the extracted entities and relationships as phrases in the question, and (ii) \emph{linking} the triplet into corresponding synonymous \texttt{subject}/\texttt{objects} or \texttt{predicate} to construct basic graph patterns (\emph{BGPs}), i.e., the SPARQL query building block.  

The phrase-based \emph{triple patterns} is a cornerstone of the \emph{BGPs} to be eventually generated, while the predicted synonyms dominate the answers' correctness. For example, the two triple patterns in Figure~\ref{fig:nlq} are connected through the same subject (\texttt{?unknown}), which represents the name of the sea. Due to the high variability of KGs' domains, \emph{question understanding} should adjust dramatically for each domain to deal with various kinds of entities/relationships connected in different ways, e.g., a paper identified by a long title to a location known by a single name. Furthermore, RDF engines lack the support for built-in mechanisms to lookup \texttt{subject}/\texttt{objects} or \texttt{predicate} based on synonyms or semantic search. For example, RDF engines cannot identify that the predicate \emph{nearestCity} is a synonym for "city on shore". Thus, forming an equivalent SPARQL query immediately for a question against an arbitrary KG is challenging for an \emph{on-demand KG QAS}.
 
Existing QASs index the target KG in advance based on synonyms, such as EDGQA~\cite{EDGQA} and gAnswer~\cite{gAnswer2018, gAnswer2014}, or build a vector space of all KG's nodes and edges to predict synonyms based on deep learning models, such as NSQA~\cite{NSQA}.
EDGQA outperformed NSQA and gAnswer in the main benchmarks for question-answering, namely LC-QuAD 1.0~\cite{LCQuAD1} and QALD-9~\cite{QALD9-018}. 
%gAnswer was ranked first in the QALD-9 challenge~\cite{QALD9-018}. 
In these systems, the preprocessing cost is proportional to the KG's size. For example in gAnswer, the preprocessing complexity is polynomial to the number of KG's vertices~\cite{gAnswer2018, gAnswer2014}. EDGQA utilizes three different systems to index the target KG, where each system indexes the KG differently. Ordinary users cannot use existing QASs on-demand due to the complexity of their preprocessing phase and its huge time. Furthermore, \emph{question understanding} in these systems utilizes semantic parsing and curate rules based on the part of speech tags, such as a noun or verb, to extract entities and relationships. For an \emph{on-demand KG QAS}, \emph{question understanding} based on curated rules is hard to generalize to a broad set of application domains.

\begin{figure}[t]
\ncp\ncp
% \small
\begin{verbatim}

1 PREFIX dbpedia:<http://dbpedia.org/resource/> 
2 SELECT ?unknown WHERE { 
3 ?unknown <http://dbpedia.org/property/outflow>
   dbpedia:Danish_straits . 
4 ?unknown <http://dbpedia.org/ontology/nearestCity> 
   dbpedia:Kaliningrad . }
\end{verbatim}
\ncp\ncp\ncp\ncp\ncp
% QID:4149
\caption{A SPARQL query finding the name of the sea into which Danish Straits flows and has Kaliningrad as one of the \emph{city} on the shore. Synonyms could be as easy as (Danish Straits, \emph{Danish\_straits}) to a more challenging ones as (flows, \emph{outflow}) or (city on shore, \emph{nearestCity}). Correct grammar is not guaranteed, e.g., "city" is used instead of "cities".
}
\label{fig:nlq}
\ncp\ncp\ncp\ncp\ncp\ncp\ncp
\end{figure}

This paper presents {\sysName}, an on-demand \underline{KG}  \underline{Q}uestion-\underline{An}swering platform. In this paper, we propose a novel formalisation of  the \emph{question understanding} and \emph{linking} problems, plus an innovative method for filtering the final answers. RDF engines index all triples in six possible ways for traditional lookup~\cite{Hexastore, TripleBit}, and provide indices for text search~\cite{quoc2019performance}. Examples for these RDF engines are Virtuoso, Stardog, and Apache Jena, which are widely used to store KGs~\cite{quoc2019performance}. To the best of our knowledge, {\sysName} is the first fully-fledged on-demand question-answering platform\footnote{\url{https://github.com/CoDS-GCS/KGQAn}} based on RDF engines' built-in indices and models trained independently of the target KG. The main paper's contributions are the following: 

\textbf{-} An inventive formalization of the \emph{question understanding} problem as a text generation task to extract phrase triple patterns (\emph{PTP}) from a question. Unlike the triple extraction models trained to construct KGs~\cite{triples2020, triples2022}, our task includes the detection of unknowns and their connections to the entities and relationships, whose phrases are explicitly mentioned in the question. We trained our task as a Seq2Seq model, where the input is a question and the output is a set of \emph{PTP}s. Our model learns automatically to distinguish between unknowns, entities, and relationships and forms them into \emph{PTP}s. {\sysName} constructs a phrase graph pattern (\emph{PGP}) from this set. 

\textbf{-} A novel Just-in-Time (JIT) linking approach to annotate the \emph{PGP}'s entities and relationships with vertices and predicates in a KG by taking advantage of the RDF engines' built-in indices and a semantic affinity model trained on general English text. {\sysName} formalizes the linking process as text search queries to an RDF engine then {\sysName} performs semantic ranking to find $V$, a list of top-k vertices matching an entity syntactically and semantically. Then, {\sysName} iterates over $V$ to fetch predicates of a certain vertex using lightweight queries executed by the RDF engine, then 
{\sysName} applies our semantic affinity model to sort them. 
%For example, {\sysName} identifies the predicate \emph{nearestCity} third after \emph{city} and \emph{locationCity} as synonyms to  "the city on the shore", and \emph{outflow} is ranked first as a synonym to flows. 
 
\textbf{-} A resourceful post-filtering method to percolate answers collected by executing the semantically equivalent queries. 
Existing QASs, such as EDGQA, adopt a filtering method that demands prior knowledge of all node types in a KG. {\sysName}, as an on-demand service, avoids this limitation by predicting the answer type of the unknowns, e.g., string, number, or date, and retrieve the node type of the variables in the generated SPARQL query. {\sysName} filters answers, whose type does not match the predicted one.                      

\textbf{-} A comprehensive evaluation against the state-of-the-art QASs using using four real KGs of different application domains, namely Microsoft Academic Graph, DBLP, DBpedia, and Yago. We used LC-QuAD 1.0  and QALD-9 benchmarks, which are commonly used to measure QASs's F1-measure. The state-of-the-art QASs demand a few hours to days of preprocessing based on the KG size. With Zero preprocessing, {\sysName} outperformed these systems in terms of F1-measure in most cases, and  question processing latency.

The paper is organized as follows. Section~\ref{sec:comp} discusses the background of QASs and their limitations. Section~\ref{sec:overview} outlines the {\sysName}'s architecture. Section~\ref{sec:triples},~\ref{sec:linking}, and~\ref{sec:exec} discuss the {\sysName}'s \emph{question understanding}, \emph{linking}, and \emph{post-filtering} methods. We discuss our comprehensive evaluation in Section~\ref{sec:results}, and related work in Section~\ref{sec:relatedwork}. 
Section~\ref{sec:conc} concludes the paper.


%Existing QASs preprocess the target KG in advance to index it based on synonyms, such as EDGQA~\cite{EDGQA} and gAnswer~\cite{gAnswer2018, gAnswer2014} or build a vector space of all KG's nodes and edges to align synonyms based on semantics, such as NSQA~\cite{NSQA}. EDGQA outperformed NSQA and gAnswer in the main benchmarks for question-answering, namely LC-QuAD 1.0~\cite{LCQuAD1} and QALD-9~\cite{QALD9-018}. gAnswer was ranked first in the QALD-9 challenge~\cite{QALD9-018}. NSQA utilizes a linking approach~\cite{nsqa_linking} based on models trained using a vector space of KG's nodes or edges, i.e., it needs full access of the KG in advance.  In these systems, the preprocessing cost is proportional to the size of the KG. For example, the time complexity of the preprocessing phase in gAnswer is polynomial to the number of KG's vertices~\cite{gAnswer2018, gAnswer2014}. EDGQA utilizes three different systems to index the target KG, where each system indexes the KG differently. Ordinary users cannot use existing QASs on-demand due to the complexity of their preprocessing phase and its huge time. Furthermore, \emph{question understanding} in these systems utilizes semantic parsing and curate rules based on the part of speech tags, such as a noun or verb, to extract entities and relationships. %Intuitively, these rule-based approaches show promising results as these systems competed for specific benchmarks that use only DBpedia, i.e., one single domain. For an \emph{on-demand KG QAS}, \emph{question understanding} based on curated rules is hard to generalize to a broad set of application domains.


%Unlike \emph{BGP}, our \emph{PGP} is an undirected graph, whose nodes are an unknown or a named entity, and edges are relation phrases. 


 %{\sysName} answers a question expeditiously on an arbitrary KG through a three-fold pipeline without any preprocessing. 

% {\sysName}  identifies synonymous vertices for an entity by searching for vertices whose label contains the entity’s phrase then sorting these vertices based on semantic affinity. For example,  {\sysName} sorts \url{http://dbpedia.org/resource/Diana,_Princess_of_Wales}, whose label is "Diana Princess of Wales" as top vertex matching “Princess Diana”.  



==> sections/old-files/introduction_reham.tex <==


 \section{Introduction}
 \label{sec:intro}

There is growing adoption of knowledge graphs (KGs) across the industry on variant domains, such as life science and media. The RDF data model is widely utilized to store KGs due to RDF's simplicity, powerful query language (SPARQL), and extensions. These extensions help in formalizing constraints and semantics on top of RDF datasets that enables inferencing and reasoning to enrich KGs with new facts. Hence, there is an explosion in the number of RDF-based KGs, which have an online service. Examples of these KGs are DBpedia ~\footnote{\url{https://dbpedia.org/sparql}} which contain structured information gathered from different Wikimedia projects, Microsoft Academic Graph~\footnote{\url{https://makg.org/}} which contains eight billion triples about scientific publications, authors, and institutions, DBLP \footnote{https://dblp.org/} which contains the information about major computer science journals and proceedings, YAGO~\footnote{\url{https://yago-knowledge.org/sparql}} which combines the information from two sources, the first source is Wikidata which is considered one of the largest general knowledge bases and the second source is schema.org which is the standard ontology of classes and relations.
More examples of knowledge graphs includes Bio2RDF~\footnote{\url{https://bio2rdf.org/sparql}}, Wikidata~\footnote{\url{https://query.wikidata.org/}}, OpenCitations \footnote{\url{https://opencitations.net/sparql}} and the UK Parliament~\footnote{\url{https://api.parliament.uk/sparql}}. 

The RDF data model represents \RDFTYPE{subject}{predicate}{object} triples, where a relationship (\texttt{predicate}) and an entity (\texttt{subject} or \texttt{object}) are identified by a URI. Forming structured SPARQL queries requires prior knowledge about the query language, the schema of the KG, as well as the exact URIs of the entities and predicates. For example, to form the query in Figure~\ref{fig:nlq}, users need to \myNum{i} be aware of the exact URIs of predicates, e.g., {\tt<\url{http://dbpedia.org/property/outflow}>}, and entities, e.g., {\tt<\url{http://dbpedia.org/resource/Danish_straits}>},  and 
\myNum{ii} identify basic graph patterns (BGP) and how the different triples are connected to each other, e.g., the two triple patterns in Figure~\ref{fig:nlq}, are connected through the same subject (?uri) which represents the name of the sea. Thus, forming a SPARQL query is challenging.

\begin{figure}[t]
% \ncp
\small
\begin{verbatim}

1 PREFIX dbpedia:<http://dbpedia.org/resource/> 
2 SELECT ?uri WHERE { 
3 ?uri <http://dbpedia.org/property/outflow>
   dbpedia:Danish_straits . 
4 ?uri <http://dbpedia.org/ontology/nearestCity> 
   dbpedia:Kaliningrad . }
\end{verbatim}
% \ncp\ncp\ncp\ncp\ncp
\caption{A SPARQL query to find the name of the sea into which Danish Straits flows and has Kaliningrad as one of the city on the shore.}
\label{fig:nlq}
% \ncp\ncp\ncp\ncp\ncp
\end{figure}

To support inexperienced users in exploring KGs easily, KG question-answering systems map a question into semantically equivalent SPARQL queries. EDGQA ~\cite{EDGQA} use a set of predefined rules to understand the question. This technique is good if it is guaranteed that the set of rules used is the complete set of rules that cover all possible English questions. Other systems access the entire KG in a preprocessing phase to build indexes and dictionaries, such as gAnswer ~\cite{gAnswer2018, gAnswer2014} and QAMP ~\cite{QAMP}.  
This preprocessing phase has two problems: 1) The complexity of the preprocessing is proportional to the size of the graph. For example, gAnswer generates dictionaries for entities and relations of almost 60 GB to answer queries on a DBpedia dataset of about 6 GB,  2) The preprocessing phase makes the system dependent on only the knowledge graph that was pre-processed, which makes the systems hard to generalize on different knowledge graphs.
% Existing systems suffer from low accuracy and high false positive rates.
NSQA and EDGQA are the top-ranked systems for QALD-9~\cite{qald9}, a widely used question answering benchmark, achieving F1-measure of 31.26 and 32 with precision 31.89 and 31.3, respectively, as reported in~\cite{ NSQA, EDGQA} which shows that there is still a big room for improvement for this specific dataset and for the KGQA problem in general. 


We developed KGQAn, a question-answering platform, to address the above challenges. Unlike existing systems, KGQAn can deal with different knowledge graphs without the need of redoing the excessive preprocessing phase or re-training any of its models. Figure ~\ref{fig:systemOverview}, shows how KGQAn interacts with different users and different endpoints where the users provide KGQAn with the question and the Endpoint they want to query and KGQAn create the SPARQL query representing the question, executes it and send the results back to the user.  KGQAn runs in three phases. In the first phase, KGQAn constructs a PGP, a graph pattern that represents the question, from the phrases in the given question. The model used for question understanding is a Sequence to sequence model, which has the ability to map sequences of different length to each other. This improves the system’s ability to deal with the long complex questions that the parser-based techniques fails to handle.


\begin{figure}
\ncp\ncp
  \centering
  \includegraphics[width=\columnwidth]{figures/Figure2.pdf}
  \ncp\ncp\ncp\ncp\ncp\ncp\ncp
\caption{Overview of KGQAn's interaction with users}
\label{fig:systemOverview}
\ncp\ncp\ncp\ncp
\end{figure}


In the second phase, KGQAn proposes Just-in-Time (JIT) approach to link phrases in the PGP with the KG. The KGQAn’s JIT approach is used to annotate the entities and relations of the PGP with vertices and predicates from the corresponding knowledge graph by taking advantage of the built-in indices in the RDF engines. Linking the entities to vertices and relations to predicates takes place using simple SPARQL queries. In order to execute these queries we need a SPARQL endpoint. KGQAn links the entity with the top vertex whose label matches the entity. Then, KGQAn gets a list of predicates connected with the vertex. Instead of searching the whole graph, we only consider the subgraph which contains our chosen vertex. Thus, this prunes the search space for the predicates. 

The simple queries are designed to take advantage of the fact that RDF engines are optimized to search for triples using subjects or objects. To select the vertices and predicates, KGQAn ranks the candidate vertices and predicates based on their semantic similarity with the entities and relations, e.g. relation "write" semantically matches predicate "author". Finally, KGQAn navigates the annotated PGP to generate the SPARQL queries with the highest score, execute them, and uses the just in time filtering technique to compares the type of the result with the predicted answer type of the question and remove results that do not match.  This eliminates the need of the pre-processing phase that gets all possible types that exist in the KG.


The contributions of this work can be summarized as follows:
\begin{itemize}
    \item We propose KGQAn, a framework that allows users to easily query multiple graphs using natural language it is trained independently of the graph, which makes it able to deal with different knowledge graphs from different domains without the need of re-training. 

    \item We mapped the question understanding problem to a text generation problem and used a sequence to sequence model to perform the extraction of triples from the question. This leverages the ability of the deep learning models to learn the structure of the text instead of using parsing-based models that miss the noun relation phrases.

    \item  We propose a Just in time  approach for linking the extracted entities and relations to vertices and predicates from the knowledge graph. This approach prunes the search space, which makes the process of relation linking more efficient. It also removes the need of building indices.
    
    
    \item We demonstrate the  performance of KGQAn on two well known benchmarks, QALD9 and LC-QUAD1.0. KGQAN achieves state-of-the-art results on QALD-9 by an improvement of 37.41\% in F1-measure and 58.98\% in precision., and it is so close to the best performance on LC-QUAD1.0.
    
    \item We demonstrate the generality of KGQAn by running the system on questions from different knowledge graphs: DBpedia, Yago, DBLP and Microsoft Academic.
\end{itemize}


The paper is organized as follows: Section~\ref{sec:comp} discusses the background of Knowledge Graph Question Answering and its limitations. Section~\ref{sec:overview} outlines an overview of the architecture of {\sysName}. Section~\ref{sec:triples},~\ref{sec:linking}, and~\ref{sec:exec} details the three phases followed by {\sysName}. Section~\ref{sec:results} shows the experimental results and Section~\ref{sec:relatedwork} discusses pre-existing related work in Knowledge Graph question answering,  followed by a final conclusion in Section~\ref{sec:conc}.


==> sections/overview_submitted.tex <==
\section{{\sysName}'s Architecture and Models}
\label{sec:overview}

The {\sysName} architecture is shown in Figure~\ref{fig:architecture} with an end-to-end demonstration using $q^E$. 
% {\sysName} utilizes different models for constructing a PGP from a question and annotating it with relevant vertices and predicates in a KG. 
The {\sysName} platform is fully implemented using \emph{Python} 3.7 and all models were trained using \emph{Pytorch} 1.11.0. Our platform supports parallel execution and filtration via multi-threading. This section highlights details of the {\sysName} models.
% used for \emph{question understanding} (\emph{QU}) and \emph{linking}.\shorten


\nsstitle{The Seq2Seq Model for QU.}  
% We are the first to define the triple patterns extraction task from a question. Thus, 
We prepared a manually annotated dataset where the input is an English question, and the output is a sequence of triple patterns. This dataset is built using 1752 questions collected from the training dataset of {\lcq}~\cite{lcquad} and {\qald}~\cite{qald9}. Our annotated dataset does not include the SPARQL queries. We only use the English questions from {\lcq} and {\qald} to annotate them. 
% Each phrase triple pattern is formed as \RDFTYPE{$Entity_i$}{Relation}{$Entity_j$}. Unlike SPARQL, our phrase triple pattern is undirected. An entity could be unknown, i.e., a variable. If an entity is a variable, then all the information about the variable will also be provided in the annotated dataset, such as the answer type and a variable identifier.
%
We defined our phrase triple pattern extraction as a text generation task, which needs an encoder-decoder seq2seq language model, such as BART~\cite{BART} and T5~\cite{T5}. We adopted BART to train a Seq2Seq Model for our task. BART showed promising performance when fine-tuned for text generation tasks. Our model is trained on a machine with one GPU with early stopping enabled, a batch size of 4, \emph{3} epochs, and the \emph{Adam} optimizer. These parameters are chosen based on our hyperparameter tuning. 

% process where we tried different values for these parameters. 

% For example, batch size values varied from 4 to 32 and the number of epochs varied from 3 to 50, and the values stated showed the best performance. 
% Our model is evaluated using the Rouge~\cite{rouge} metric. Rouge is one of the metrics that can be used to evaluate the performance of text generation models. The quality of the model output is determined by comparing it to the target output specified in the datasets. In our model, the Rouge is calculated by comparing the output of the decoder to the target triples expected.\shorten

\nsstitle{The Answer Type and Semantic Affinity Model.}
{\sysName} predicts the answer type at a \textit{default} and \textit{semantic} granularity. To predict the \textit{default} data type, i.e., date, numerical, boolean, and string, we trained a three-layer neural network. We used the {\qald} dataset as its questions are annotated with their answer data type. In our model, the first layer consists of 100 units with Relu activation function, the second layer consists of 50 units with Relu activation function, and the last layer consists of 4 units with softmax activation function. The optimizer used is a stochastic gradient descent with 0.01 learning rate. For predicting \textit{semantic} data types, we used a heuristic based on a constituency parser. The current implementation used AllenNLP constituency parser. 
For semantic affinity model, we used Glove, which provides a set of pre-trained models \footnote{\url{https://nlp.stanford.edu/projects/glove/}}. The current implementation used the model trained on six billion tokens and a vocabulary dictionary that contains 400K words, with a vector size 300. 
\highlight{The {\sysName} code is available here \footnote{https://gitfront.io/r/user-2881158/9ED3DRTbntgA/KGQAN/}}

\begin{figure}
\ncp\ncp\ncp
  \centering
  \includegraphics[width=\columnwidth]{figures/KGQAnArchitecture.pdf}
  \ncp\ncp\ncp\ncp\ncp\ncp\ncp
\caption{
{\sysName}'s architecture includes three phases: a) the PGP construction using our Seq2Seq model, b) the JIT linking to annotate the PGP with relevant vertices and predicates in a KG, and c) the execution and post-filtering.

}
\label{fig:architecture}
\ncp\ncp\ncp\ncp\ncp\ncp\ncp
\end{figure}



% \nsstitle{Linking PGP to a KG.}
% We developed a semantic affinity model for our JIT Linking and filtering approach. 
% We utilized mainly word embeddings to calculate the cosine similarity between the embeddings for a pair of words. 
% % Finally, we average the cosine similarity of all pairs.  
% For word embeddings, we use Glove, which provides a set of pre-trained models \footnote{\url{https://nlp.stanford.edu/projects/glove/}}. The current implementation used the model trained on six billion tokens and a vocabulary dictionary that contains 400K words, with a vector size 300. We use the character-level embeddings to deal with words not included in the WE pre-trained model, i.e., \textit{unknowns}. For the character level embedding, we used \emph{Chars2Vec}~\footnote{\url{https://github.com/IntuitionEngineeringTeam/chars2vec}}, where the similarity of word spellings is captured by the distance metric between the embeddings.





==> sections/related_work_old.tex <==
\section{Related Work }
\label{sec:relatedwork}

==========

\hl{Moved here from intro}

 Unlike the triple extraction models trained to construct KGs~\cite{triples2020, triples2022}, our task includes the detection of unknowns and their connections to entities and relationships, whose phrases are explicitly mentioned in the question. 
 
 


==========


In knowledge graph based question answering, both natural understanding and linking are required. Filtration may additionally be used. Systems may be end-to-end performing the two steps in a single swoop, or they may alternatively be modular. 
Systems that employ neural networks to generate end-to-end pipelines are typically knowledge graph specific. For example, \cite{Large_Scale_Bordes} employ a memory network which includes knowledge graph entities and edges. For a new knowledge graph to be queried, the nodes of the new graph must be associated to which existing nodes in this network.

Early work in KBQA focused on solving simple questions containing a single relation. The early ideas included using semantic parsing techniques to convert the given question to a logical form \cite{BerantCFL13}\cite{YihCHG15} or SPARQL queries \cite{BastH15}. Other systems used information retrieval techniques to solve the problem, \cite{YaoD14}  gets a set of possible answer candidates using information extraction methods, then they use different methods to analyze this set of candidates and rank them. 
Systems that are modular also rely on information from a particular knowledge graph for question parsing. For example, \cite{WuFofe}  employ FOFE-nets (Fixed-size Ordinally Forgetting Encoding with feed forward neural networks) for multiple steps of their pipeline: topic subject discovery, entity linking, relation detection and constraint detection. Each of these FOFE-nets is trained on either Freebase or an extract of Freebase. \cite{WuFofe}. Unlike {\sysName}, these systems can not handle complex questions which contains more than one triple. Most of the recent work are graph driven systems, which attempts to construct sub-graph from the question to query the KG, include top-performing systems such as gAnswer ~\cite{gAnswer2018, gAnswer2014}, QAmp \cite{QAMP} and EDGQA \cite{EDGQA}. 
These systems employ the graph to construct SPARQL queries to be executed to return the answers to the user.


\textbf{Semantic parsing based systems} are the systems which depend on NLP semantic parsing model in the question understanding step. Examples of these systems are \cite{gAnswer2018}, \cite{NSQA}, \cite{ChenLHQ20}, and \cite{LanJ20}. 
In \cite{ChenLHQ20} the query building module is enhanced to eliminate the generation of noisy and wrong structured queries that affected the performance of previous systems. They divide the query generation into two parts, the first part predicts the correct structure of the query given the question as an input, then this structure is used to generate the candidate queries. 
\cite{LanJ20} is a semantic based approach that started concentrating on complex questions, by adding constraints to the query graph. The query graph is generated using a semantic parsing method, and the constraints are added during the construction of the query graph. This makes the process of generating the query graph more efficient. Although these systems have a better ability to work with complex questions than early systems, they are not effective when dealing with long questions where parsers sometimes struggle to deal with. {\sysName} solves this problem by using the Seq2seq model for question understanding.

\textbf{Information Retrieval systems} are the systems that depend on information retrieval techniques to perform the question understanding task, such as \cite{WangNNX21} and \cite{YaoD14}. \cite{WangNNX21} uses inverted indices for entities and predicates, then TF-IDF method is used to retrieve the candidates. These candidates are re-ranked using BERT-based neural networks in an optimized way. These systems have comparable results to the semantic-parsing based systems, and they also share the same problem when the questions are long. 

\textbf{General systems}: some recent work took initial steps to generalize Knowledge Base Question Answering systems such as \cite{sygma}, \cite{biosoda} and \cite{qanswerKG}.
{SYGMA} \cite{sygma} developed their approach to work with  Dbpedia and Wikidata. In the question understanding step, AMR parsing is used to understand the question, which is a semantic representation language based on PropBank. Then the generated AMR is converted to lambda calculus expressions. For the linking step, these lambda expressions are transformed to KB specific lambda expressions with the help of pre-existing techniques for entity and relation linking. For entity linking, BLINK \cite{blink} is used with  an entity dictionary of  5.9M English Wikipedia entities, mapped to their corresponding Wikidata and DBpedia entities. For Relation Linking, \cite{nsqa_linking}, they used AMR based relation linking approach where they use models trained specifically for each KG. Therefore, to support a new KG, they have to re-train the models used in their AMR based relation linking technique. Lastly, the KB specific lambda expression is transformed to SPARQL using another set of pre-defined transformations.
{\sysName} is a step towards moving to a more general system where, unlike SYGMA, we don’t need to train different models to support different KGs. Moreover, there is no need in KGQAn to have a large entity dictionary for all entities in the supported KGs.

Bio-SODA \cite{biosoda} is a QA system that targets scientific knowledge graphs. It focuses on scientific datasets where there is no available training data. The motivation to this work is that the existing systems do not generalize well to different KGs because it has strong coupling with the knowledge graphs they were developed for. It also does not generalize well to other domains, such as the scientific domain. Bio-SODA first needs to pre-process the target knowledge graph. This pre-processing phase includes building indices from the target RDF store (KG) so it can be further used in the lookup step in the next phase. The inverted indices were saved as relational databases for fast lookups.
After building the required inverted index, Bio-SODA can start processing the questions. First, the question tokens are sent to the inverted index for the lookup process. The output of the lookup process are the URI of the token, the page rank score, class and property name.  Then the returned candidate tokens are ranked based on syntactic similarity, semantic similarity and node centrality in the KG. The highly ranked tokens are used to construct the candidate query graphs. Then the query graphs are ranked depending on their relevance to the user question. Finally, the SPARQL query is built from query graphs and the answers are returned to the user. Bio-SODA approach concentrated on replacing the linking tools that are trained for a specific KG, e.g. DBpedia as these approaches can only deal with the KG they are trained on. They replace these modules through building their own index. So they still require having a pre-processing phase before dealing with a new KG. On the other hand, {\sysName} can deal with a new KG without having any pre-processing step thanks to its Just-in-time linking module. 

QAnswer KG \cite{qanswerKG} divided the KGQA pipeline into 4 steps: Query Expansion, Query Construction, Query Ranking, and Answer Decision. but before it starts working on questions from a specific knowledge graph, an indexing step is required, where the dataset under consideration is uploaded and indexed. For the first step, all possible n-grams from the question are extracted and mapped to resources from the KG using the index. In the second step, all possible SPARQL queries are created by generating all combinations from the mapped resource, Then the generated SPARQL queries are ranked using a pre-trained machine learning component. For the last step, a model is used to calculate the confidence of the highly ranked answers to return the highest ranked answer with a good confidence.

Although Bio-SODA and QAnswer KG can generalize without the need to change in the codebase, the pre-processing phase will need to be repeated with each new knowledge graph. On the other hand, KGQAn can generalize without the need to change the code base and without any pre-processing phase, so nothing needs to be performed before working on a new knowledge graph. 


==> sections/seq2seq_old.tex <==
\section{{\sysName} Question Understanding}
\label{sec:triples}

In this section, we explain the first step of our system, where we convert the input natural language question to a set of relation triples which then will be converted to a PGP representing the question. To achieve that, we formulated the problem differently, instead of relying on parsers to extract the entities and relations from the question, we mapped the problem to a text generation problem and adopted a Sequence to Sequence \cite{seq2seq} model (referred to as Seq2Seq) to solve it. The problem is formulated as follows: Given a question q = ($q_1, q_2, q_3, ... , q_n$) where $q_i$ is the word of the question in position i, it is required to get a list of triples from it T = \{$t_1, t_2, ... t_n$\} where each $t_i$ = <Subject; Predicate; Object> and each of the tokens are extracted from the given question. 

\begin{definition}[Phrase Graph Pattern (PGP)]
A Phrase Graph Pattern (PGP) is an undirected graph $P = (N, E)$, where $N$ is a set of nodes and $E$ is a set of edges, representing the understanding of the question. Each node $n_i \in N$ is associated with a label, and a type to indicate if this node is an unknown (variable) or an entity. Each edge $e_i \in E$ is associated with a label. 
\end{definition}



\subsection{Question to PGP}
Question understanding can be mapped to a text to graph generation task, where the input is the question (q) and the output is a phrase graph pattern (PGP) representing the question. Recent graph based system rely on parser-based techniques to do this mapping, due to the limitation of these techniques as shown in Section~\ref{sec:comp}.4. To solve these challenges, {\sysName} used a technique that depends on Seq2Seq model instead of parsers. The motivation for that was the ability of the Seq2Seq models to work on sentences (sequences) with arbitrary length.

In order to use the Seq2Seq model to solve the text to graph task, we divided the task into two steps: text to relation triples followed by a post-processing step to create the graph from the triples. Text to relation triples is a crucial task for KG construction, as a result there has been some work to tackle it such as: \cite{triples2020} and \cite{triples2022}. In our case, the question to relation triples patterns is slightly different because of the difference in inputs and outputs. Our input is a question, not a normal English sentence. Questions have a high degree of ambiguity due to the lack of context and unclarity of unknowns. Our output is a triple pattern not a normal triple, because there exists a variable (unknown) that should be predicted. Another difference between the two tasks is the fact that in our case, the components of the predicted triple pattern should be extracted from the question itself (input text), while in the text to relation triples task, the relation are chosen from a pre-defined list of relations which map the relation prediction to a relation classification task. Due to these differences, solutions used for text to relation triples task cannot be used for question to triple patterns task.\shorten

\subsection{Triple Patterns Extraction Model}
Our triple pattern extraction model is a pre-trained language model following the encoder-decoder architecture, where both the encoder and decoder are based on Transformers\cite{transformer}. Since this model is independent of the graph, as we do not provide the model with any knowledge graph specific information before giving it the inputs. As shown in the Figure ~\ref{fig:Seq2Seq}, to train our model, first, we compute the embeddings of the question and send it to the encoder, the encoder propagates all the information from the question words and creates a representation of the question that encapsulates the information of the question, we refer to this representation as encoder vector. Then we compute the embeddings of the transformed sequence of the triple patterns and send it to the decoder along with the encoder vector. The target from the training is for the decoder to predict a sequence similar to its input. The training takes place in the form of a sequence of time steps where in each time step a new word of the output is generated as shown in Equation~\ref{eq:decoder}. For the first time step, the generated word depend on the encoder vector $x$. For each subsequent time step, the generated word depends on the encoder vector $x$ and all previous generated words from the output sequence $y_i$. After the training completes, we save the trained model, so it can be later used.

The set of words that the decoder should predict the target words from is the words of the question, the symbols used for encoding and the unknown variable, this prunes the search space for the decoder as it is predicting a word from a well-defined set of words and not from all English vocabulary.
As shown in Figure~\ref{fig:Seq2Seq}, the model is trained to neglect the question word and replace it with the variable we are asking about. It also extracts the entities in the same way it exists in the question. While for the relation phrases, the noun relation phrases are directly extracted from the question. While the verb relation phrases are extracted in their infinitive form.  
The set of triples should be the input to the decoder, since we need to extract it from the question. But we can't directly use it as an input to the decoder, as the decoder only accepts sequences. One way to convert the triples to a sequence is to simply merge all triples in one single string. Although this option is good and easy to implement, it will not be easy to restore the triples again from the sequence as there is no clear limits on where triples start or end as the triple can contain arbitrary number of words. That's why we used another approach as shown in equation ~\ref{eq:predecoder}, the transformation function $F$ merges the triples while using pre-defined set of symbols to separate the different components of the triple. As shown in the decoder input in Figure~\ref{fig:Seq2Seq}, we use (e1) to indicate the start of the triple and the first entity which can either be an entity or the unknown, (r) indicates the predicate in the triple and (e2) indicates the second entity in the triple. With the help of this encoding, we can use the output of the decoder to create the PGP as the different triples and the components of each triple can be easily separated from each other.

\begin{figure}
% \ncp\ncp
  \centering
  \includegraphics[width=\columnwidth]{figures/seq2seqModel.pdf}
%   \ncp\ncp
\caption{{Architecture of Sequence-to-Sequence model used for Question Understanding }}
\label{fig:Seq2Seq}
% \ncp\ncp
\end{figure}

\begin{equation}
    y = F(T) 
    \label{eq:predecoder}
\end{equation}
\begin{equation}
    P(y|x) = P(y_1, x) P(y_2|y_1, x). . . . P(y_t|y_{t-1}, y_{t-2}, ... , y_1, x) 
    \label{eq:decoder}
\end{equation}


\subsection{The Answer Type Prediction Model}
Since our graph contains unknown nodes, we developed an answer type prediction module, which specifies the answer data type and answer type of the unknown node which will be later used to filter the answers returned to the user.

We deploy a two-step process to predict the type of the answer. The input to the module is a natural language question (q) and the output is a set of answer data type and answer type. The answer data types are predicted using a supervised classification model, and the answer type is predicted only if the answer data type is a string using a heuristic. Therefore, the output of this module is a pair ($answer_{dtype}$, $answer_{stype}$) such that:

$answer_{dtype} \in \{Numeric, Date, String, Boolean\}$ 

$answer_{stype}$ = " ", if $answer_{dtype} \notin $ \{String\}

else $answer_{stype}$ = NOUN, where NOUN is the first noun after the question word

To train the supervised classification model for predicting the answer data type, we used the training set of data from {\qald} benchmark, where the English question text was given as the input to a model and the answer data type attributes as their corresponding targets. We used {\qald} test set for testing the performance of the model. We pre-processed the question text using scikit-learn\footnote{https://scikit-learn.org/} CountVectorizer to extract and represent features of the input by transforming the corpora of question text into a vector of token counts and the targets were pre-processed using scikit-learn LabelEncoders. We experimented on four models: support vector machine, Random Forest classifier, Multi-layer Perceptron and deep neural network model. We trained the models independently and after testing them, we found the deep neural network to be the best performing model. Therefore, it was chosen to be used within {\sysName}.

The answer datatype prediction is useful for the Numeric, Date and Boolean questions as the likelihood of appearance of such types in the knowledge graph is not high unlike the String type. There is a big variety of different contexts (e.g. person, place, language, etc.) in string results, and to further identify which  subset of the list of strings we want, we developed a second step to predict the answer type of the unknown. {\color{red} @Reham please add more details about the rules.}
This step uses the following heuristic, with high probability, the first noun after the question word in a question is the answer type. For instance, for a question: "In which city is the headquarters of Air China?", the answer type would be "city" which is the first noun after the question word "which". This was implemented using AllenNLP \footnote{\url{https://allenai.org/allennlp}} pre-trained constituency parser. The constituency parser returns the structure of a question, then we go through the result till we reach the first noun.

\subsection{Integrating Trained Model with {\sysName}}
Finally, we use the trained triples patterns extraction model and the predicted pair of answer type and answer data type to create the PGP representing the question. {\sysName} uses the trained model by sending the natural language question to the model as input, the model then outputs the predicted triple patterns from this question. Starting from the section, we will show the output of each phase on our running example. The output of the triple pattern extraction model are the two triple patterns \textit{(Danish Straits, flow, ?unknown)} and \textit{(Kaliningrad, city on shore, ?unknown)}. Then these extracted triple patterns will be used to construct the PGP. For each triple $t_i$, we separate its three components: Subject, Predicate and Object, for the subject and object, first we check if there is a node with a similar label in the graph. If it exists then we return it as our first node, if it does not exist then we create a new node with this label and return it as our first node. After adding the nodes for the subject and the object, we add a related between them with the label as the Predicate. By repeating this process for all triples, we end up with the constructed PGP. After constructing the PGP, the unknown node will be updated with the answer data type and the answer type. Currently, {\sysName} can deal with a maximum of two triples, with one unknown. The PGP generated from these triples has a star graph structure.
Following the categorization of questions in \cite{lcquad2}, {\sysName} can support the following types of questions: single fact, single fact with type, Multi-fact and Boolean questions. These types of questions map to a star graph structure.

==> tables/Hyperparameters_FilteringModel.tex <==
\begin{table}[t]% h asks to places the floating element [h]ere.
%   \ncp\ncp
  \caption{Filtration Model Hyperparameters}
%   \ncp\ncp\ncp\ncp
   \label{tab:filter_parameters}
    \begin{tabular}{lc}
        \hline
        \textbf{Parameter}&{\textbf{Value}} \\
        \hline
        Batch Size & 40  \\
        Optimizer & SGD \\
        Learning Rate & 0.01 \\
        Momentum & 0.9 \\
        Number of Epochs & 150 \\
        Activation Function & relu  \\ \cline{1-2}\hline
    \end{tabular}
\end{table}


==> tables/ablation_score.tex <==
\begin{table}[t]% h asks to places the floating element [h]ere.
\ncp\ncp
     \caption{The KGQAn performance with and without filtration}
     \ncp\ncp\ncp\ncp
  \label{tab:filtration}
\begin{center}
    \begin{tabular}{l{1.78cm} p{1.2cm} p{1.2cm} p{0.8cm} p{1.7cm}|}
\hline
 \textbf{Dataset}&\textbf{Setting}&\textbf{Precision} &\textbf{Recall}&\textbf{Macro F1} \\ 
  \hline
  QALD-9&{Without Filter} &{27.70} &{42.47} &{33.53} \\
  \Block &{With Filter} &49.76 &39.39 &\textbf{43.97} \\ 
  \Block LCQuAD-1.0&{Without Filter} &48.95 &49.54 &49.23 \\
  \Block &{With Filter} &58.17 &47.22 &\textbf{52.13}\\ 
  
 \hline
\end{tabular}
\end{center}
% \label{tab:multicol}
\end{table}


% \begin{table}[b]% h asks to places the floating element [h]ere.
%      \caption{Evaluating KGQAn performance with and without filtration}
%   \label{tab:filtration}
% \begin{center}
%     \begin{tabular}{|p{1.78cm} |p{2cm}|p{1.2cm}|p{0.8cm}|p{1.3cm}|}
% \hline
%  \textbf{Dataset}&\textbf{Setting}&\textbf{Precision} &\textbf{Recall}&\textbf{Macro F1} \\ 
%   \hline
%   QALD-9&{Without Filter} &{27.7} &{42.47} &{33.53} \\ 
%   \hline

%   \Block &{With Filter} &49.76 &39.39 &\textbf{43.97} \\ 
%   \hline
%   \Block LCQuAD-1.0&{Without Filter} &48.95 &49.54 &49.23 \\   
%   \hline
%   \Block &{With Filter} &58.17 &47.22 &\textbf{52.13}\\ 
  
%  \hline
% \end{tabular}
% \end{center}
% \label{tab:multicol}
% \end{table}

==> tables/ablation_time.tex <==
% \begin{table}[h]% h asks to places the floating element [h]ere.
%      \ncp\ncp
%      \caption{Average time taken by the system to answer a question in QALD-9 and LCQuAD-1.0 in seconds}
%      \ncp\ncp\ncp\ncp\ncp\ncp
%   \label{tab:filtration_time}
%         \begin{tabular}{lccc}
%       \hline
%         \textbf{Dataset}&{\textbf{Without filtration}}&{\textbf{With filtration}}\\
%         \hline
%         QALD-9    	& 10.76               & 13.44\\ 
%         LCQuAD-1.0      & 16.20               &16.76\\ \hline
%         \end{tabular}
% \end{table}

==> tables/datasets.tex <==
\begin{table}[t] 
% \ncp\ncp
% h asks to places the floating element [h]ere.
  \caption{The used benchmarks and size of the KGs}
%   \ncp\ncp\ncp
  \label{tab:dataset}
    \begin{tabular}{lccc}
        \hline
        \textbf{Question set}&{\textbf{\#Questions}}&{\textbf{KG}}&{\textbf{\#Triples}}\\
        \hline
        {\qald} &  150 & Dbpedia-10  & 13B\\
        {\lcq} & 1000 & Dbpedia-04 & 11.5B\\
        YAGO-Bench &50& YAGO-4 &2B\\
        DBLP-Bench & 50 & DBLP&252M\\ 
        MAG-Bench & 18 & MAG&8B\\ \cline{1-2}\hline
    \end{tabular}
% \ncp\ncp\ncp\ncp
\end{table}

%        MS Academic & 18 & \\

==> tables/entity_linking.tex <==
\begin{table}[t]
 \caption{Comparison between EDGQA and {\sysName} in Entity Linking  for LCQUAD Dataset}
  \label{tab:enlinking}
        \begin{tabular}{lccc}
        \hline
        \textbf{Systems}&{\textbf{Precision}} &{\textbf{Recall}} &{\textbf{Macro F1}} \\
        \hline
        EDGQA   	&    73.85      &  68.75       &  71.2    \\ 
        % EDGQA   	&     73.1      &  68.05      &  70.5    \\ \hline
        KGQAn   &    61.68     &  52.26 & 55.38 \\ \cline{1-4}\hline 
        \end{tabular}
\end{table}

==> tables/generality_results.tex <==
\begin{table}[t]
\ncp\ncp
 \caption{Comparing the results of {\sysName} with existing Systems using different knowledge graphs}
 \ncp\ncp\ncp\ncp
  \label{tab:general}
        \begin{tabular}{lccc}
        \hline
             & {\textbf{KGQAn}} & {\textbf{EDGQA}}  & {\textbf{GAnswer}} \\
        \hline
        QALD 9  	&  43.97  &  32.00   & 29.81 \\
        LCQUAD 1.0 	&   52.13   & 53.10   & 09.25 \\
        YAGO   	&     39.39          &     24.80 & 41.80\\ 
        DBLP   &    39.20           &      20.00  & 0.00 \\ 
        MS Academic   	&    24.24   &      & \\ \cline{1-4}\hline 
        \end{tabular}
\ncp\ncp\ncp\ncp
\end{table}

%27.77

==> tables/hyperparameters.tex <==
\begin{table}[t]% h asks to places the floating element [h]ere.
%   \ncp\ncp
  \caption{Triples Generation Model Hyper parameters}
%   \ncp\ncp\ncp\ncp
   \label{tab:parameters}
    \begin{tabular}{lc}
        \hline
        \textbf{Parameter}&{\textbf{Value}} \\ \hline
        Batch Size & 4  \\
        Optimizer & Adam \\
        Learning Rate & 0.0005 \\
        Number of Epochs & 3 \\
        Activation Function & gelu  \\ \cline{1-2}\hline
    \end{tabular}
\end{table}

==> tables/language_models.tex <==
\begin{table}[t]% h asks to places the floating element [h]ere.
  \ncp\ncp
 \caption{Testing the overall performance of {\sysName} by altering one step in the pipeline. $\myNum{i}$Replacing the language model used in question understanding from BART to GPT-3, $\myNum{ii}$ replacing the semantic affinity model used in linking and filtration with GPT-3 embeddings. {\sysName} achieves comparable performance in the two cases}
  \ncp\ncp \ncp\ncp\ncp\ncp
  \label{tab:languagemodels}
  \centering       \begin{tabular}{cp{1.5cm}p{1.5cm}p{1.5cm}}
        \hline 
                % &\textbf{ \shortstack { QU BART \\ Affinity WE}} & \textbf{\shortstack { QU GPT-3 \\ Affinity WE}} & \textbf{\shortstack { QU BART \\ Affinity GPT-3}}\\
        \textbf{Benchmarks}&\textbf{QU BART + Affinity WE} & \textbf{GPT-3 QU + Affinity WE} & \textbf{QU BART + GPT-3 Affinity}\\
        \hline
        {\qald} & \textbf{43.99} & 41.00 & 41.85 \\
        {\lcq} & 52.03 & \textbf{52.79} & 51.96\\
        YAGO & \textbf{55.62} & 54.62 & 55.02 \\
        DBLP & \textbf{54.78}  & 54.21 & \\ 
        MAG &  \textbf{50.04} & 49.26 & 39.2\\ 
        \hline
\end{tabular}
\end{table}


==> tables/lcquad_results.tex <==
\begin{table}[t]% h asks to places the floating element [h]ere.
 \caption{Evaluating LCQuAD-1.0 Testing Questions (1000 Questions)}
  \label{tab:lcquad}
        \begin{tabular}{|c|c|c|c|}
       \hline
        \textbf{Systems}&{\textbf{Precision}} &{\textbf{Recall}} &{\textbf{Macro F1}} \\
        \hline
        QAMP    	& 25               & 50                        & 33 \\ \hline
        WDAqua      & 22               & 38                        & 28\\ \hline
        NSQA   	& 44.76              & 45.82                       & 44.45  \\ \hline
        EDGQA   	& 50.5              & 56                      & 53.1 \\ \hline 
        KGQAn   & \textbf{58.17}       &  47.22    &  52.13 \\ \cline{1-4}\hline
        \end{tabular}
\end{table}

==> tables/overallTime.tex <==
\begin{table}[t]
%  \ncp\ncp
 \caption{Comparison between EDGQA and {\sysName} in terms of time taken to run the benchmarks}
%   \ncp\ncp \ncp\ncp
  \label{tab:overallTime}
        \begin{tabular}{lccccc}
        \hline
        \textbf{Systems}&{\textbf{{\qald}}} &{\textbf{{\lcq}}} &{\textbf{YAGO}} &{\textbf{DBLP}}&{\textbf{MAG}} \\
        \hline
        gAnswer   &   15 min      &  10 hrs   & 5 min & 5 min &\\
        EDGQA & 30 min & 3 hrs 15 min & 5 min & 5 min &\\
        {\sysName} (ours)& 17 min & 2 hrs 8 mins & 5 min & 5 min &\\
        \cline{1-4}\hline 
        \end{tabular}
        %  \ncp\ncp
\end{table}

==> tables/pred1_uris.tex <==
\begin{table}[t]% h asks to places the floating element [h]ere.
  \caption{Top-k predicates matching the relation "city on shore"}
   \label{tab:predicate1}
    \begin{tabular}{|c|c|}
   \hline
    \textbf{Predicate}&{\textbf{Score}} \\
    \hline
    http://dbpedia.org/property/nearestCity & 0.506  \\
    \hline
    http://dbpedia.org/property/cities & 0.501 \\
    \hline
    \end{tabular}
\end{table}

==> tables/pred2_uris.tex <==
\begin{table}[t]% h asks to places the floating element [h]ere.
  \caption{Top-k predicates matching the relation "flows"}
  \label{tab:predicate2}
    \begin{tabular}{|c|c|}
       \hline
    \textbf{Predicate}&{\textbf{Score}} \\
    \hline
    http://dbpedia.org/property/outflow & 0.587  \\
    \hline
    \end{tabular}
\end{table}

==> tables/preprocessing_time.tex <==
% \begin{table}[t]
% %  \ncp\ncp
%  \caption{Time taken by systems to pre-process different KGs}
% %   \ncp\ncp\ncp
%   \label{tab:preprocessing}
%         \begin{tabular}{lcccc}
%       \hline
%         \textbf{KG}&{\textbf{EDGQA}} & {\textbf{Index}} &{\textbf{gAnswer}} & {\textbf{Index}}\\
%         \hline
%         DBLP & 2.5 hrs & 1.6G & 2.6 hrs & 9.4G\\ 
%         LCQuAD 1.0 &   3.1 hrs &  1.7G  & 3.1 hrs & 6.5G \\ 
%         QALD-9   	&   3.8 hrs & 1.9G & 3.9 hrs & 8.6G \\ 
%         YAGO      &       3.9 hrs    &   2.1G & 2.5 hrs & 4G\\
%         MAG      & &  &  & \\ \hline 
%         \end{tabular}
% \end{table}

\begin{table*}[t]% h asks to places the floating element [h]ere.
%   \ncp\ncp
 \caption{Time taken by systems to pre-process different KGs}
%   \ncp\ncp \ncp\ncp
 \label{tab:preprocessing}
        \begin{tabular}{lcccccc}
        \hline
         \multicolumn{2}{c}{}&\multicolumn{3}{c}{\textbf{EDGQA}} & \multicolumn{2}{c}{\textbf{gAnswer}} \\
        \textbf{Graph}&{\textbf{\#Triples (B)}} &{\textbf{Load Time(hrs)}} & {\textbf{Index Time(min)}} &{\textbf{Index Size(G)}} &{\textbf{Time(hrs)}} &{\textbf{Index Size(G)}}\\
        \hline
        LCQuAD-1.0& 9.50 & 6.14 & 6 & 1.70 & 2.28 & 6.60\\ 
        QALD-9 & 13.00 & 6.40 & 7 & 1.80 & 2.86 & 8.60\\
        YAGO  & 2.00 & 6.73 & 9 & 2.00 & 1.81 & 4.10\\ 
        DBLP & 0.25 & 4.56 & 16 & 1.60 & 1.91 & 5.20 \\ 
        MAG & 8.00 & - & - & - & - & -\\ \hline
\end{tabular}
        %  \ncp\ncp \ncp\ncp
\end{table*}




==> tables/qald9_results.tex <==
\begin{table}[t]% h asks to places the floating element [h]ere.
%   \ncp\ncp
 \caption{Results for standard benchmarks: QALD-9 (150 questions) and LCQuAD-1.0 (1000 questions).}
%   \ncp\ncp \ncp\ncp
 \label{tab:qald_lcquad}
        \begin{tabular}{lcccccc}
        \hline
         & \multicolumn{3}{c}{\textbf{{\qald}}} & \multicolumn{3}{c}{\textbf{{\lcq}}} \\
        \textbf{System}&{\textbf{P}} &{\textbf{R}} &{\textbf{F1}} &{\textbf{P}} &{\textbf{R}} &{\textbf{F1}} \\
        \hline
        QAMP    	& -  &   -   &   -   &  25.00               & 50.00                        & 33.00 \\ 
        gAnswer 	& 29.34               & 32.68                         & 29.81 &    -    &    -    &    -    \\ 
        % WDAqua    	& 26.09               & 26.70                        & 24.99 & 22.00               & 38.00                        & 28.00\\ 
        NSQA   	& 31.89               & 32.05                       & 31.26  & 44.76              & 45.82                       & 44.45 \\ 
        EDGQA   	& 31.30              & 40.30                       & 32.00 & 50.50              & \textbf{56.00}                      & \textbf{53.10}\\  \hline
        \textbf{{\sysName}-F }    & 27.70   & \textbf{41.81}     &  33.32   & 48.85       &  49.46    &  49.15 \\        
        \textbf{{\sysName}+F}    & \textbf{49.81}        & 39.39     &  \textbf{43.99}   & \textbf{58.07}       &  47.12    &  52.03 \\ \hline 
        \end{tabular}
        %  \ncp\ncp \ncp\ncp
\end{table}


% \begin{table*}[t]% h asks to places the floating element [h]ere.
% %   \ncp\ncp
%  \caption{Results for standard benchmarks QALD-9 and LCQuAD-1.0}
% %   \ncp\ncp \ncp\ncp
%  \label{tab:qald_lcquad}
%         \begin{tabular}{lcccccc}
%         \hline
%          & \multicolumn{3}{c}{\textbf{{\qald}, 150 questions}} & \multicolumn{3}{c}{\textbf{{\lcq}, 1000 questions}} \\
%         \textbf{System}&{\textbf{Precision}} &{\textbf{Recall}} &{\textbf{Macro F1}} &{\textbf{Precision}} &{\textbf{Recall}} &{\textbf{Macro F1}} \\
%         \hline
%         QAMP    	& -  &   -   &   -   &  25.00               & 50.00                        & 33.00 \\ 
%         gAnswer 	& 29.34               & 32.68                         & 29.81 &    -    &    -    &    -    \\ 
%         % WDAqua    	& 26.09               & 26.70                        & 24.99 & 22.00               & 38.00                        & 28.00\\ 
%         NSQA   	& 31.89               & 32.05                       & 31.26  & 44.76              & 45.82                       & 44.45 \\ 
%         EDGQA   	& 31.30              & 40.30                       & 32.00 & 50.50              & \textbf{56.00}                      & \textbf{53.10}\\  \hline
%         \textbf{{\sysName} } (without Filtration)   & 27.70   & \textbf{41.81}     &  33.32   & 48.95       &  49.46    &  49.15 \\        
%         \textbf{{\sysName}} (with Filtration)   & \textbf{49.81}        & 39.39     &  \textbf{43.99}   & \textbf{58.07}       &  47.12    &  52.03 \\ \hline 
%         \end{tabular}
%         %  \ncp\ncp \ncp\ncp
% \end{table*}




==> tables/questionUnderstanding.tex <==
\begin{table*}[t]% h asks to places the floating element [h]ere.
%   \ncp\ncp
 \caption{Comparison of number of questions failed due to Question Understanding over total number of questions failed by the systems on different KGs}
%   \ncp\ncp \ncp\ncp
 \label{tab:qufailed}
        \begin{tabular}{lccc}
        \hline
         & \multicolumn{3}{c}{\textbf{Questions failed in question understanding/Total questions with Recall = 0}}\\
        \textbf{System}&{\textbf{{\qald}, 150 questions}} &{\textbf{YAGO, 100 questions}} &{\textbf{DBLP, 100 questions}} \\
        \hline
        gAnswer & 54/128 & 28/65 & 89/100 \\ 
        EDGQA   & 44/88 & 33/57 & 49/92 \\ 
        {\sysName} (ours)& 36/88 & 8/32 & 7/14\\  \hline
\end{tabular}
        %  \ncp\ncp \ncp\ncp
\end{table*}




==> tables/recall_systems.tex <==
\begin{table*}[t]% h asks to places the floating element [h]ere.
%   \ncp\ncp
 \caption{Comparison of number of questions solved by the given systems with Recall=0, Recall=1 and Recall between 0 and 1 over standard benchmarks QALD-9 and LCQuAD-1.0}
%   \ncp\ncp \ncp\ncp
 \label{tab:recall}
        \begin{tabular}{lcccccc}
        \hline
         & \multicolumn{3}{c}{\textbf{{\qald}, 150 questions}} & \multicolumn{3}{c}{\textbf{{\lcq}, 1000 questions}} \\
        \textbf{System}&{\textbf{R=0}} &{\textbf{R=1}} &{\textbf{0 < R < 1}} &{\textbf{R=0}} &{\textbf{R=1}} &{\textbf{0 < R < 1}} \\
        \hline
        gAnswer & 128  & 19 & 3 & 980 & 16 & 4 \\ 
        EDGQA   &  88  & 59 & 3 & 418 & 549 & 33 \\ 
        {\sysName} (ours) & 88 & 57 & 5 & 506 & 456 & 38\\  \hline
\end{tabular}
        %  \ncp\ncp \ncp\ncp
\end{table*}




==> tables/relation_linking.tex <==
\begin{table*}[t]% h asks to places the floating element [h]ere.
%   \ncp\ncp
 \caption{Comparison between EDGQA and {\sysName} in entity and relation linking for LCQuAD-1.0}
%   \ncp\ncp\ncp\ncp
 \label{tab:rellinking}
        \begin{tabular}{lccccccc}
        \hline
         & \multicolumn{3}{c}{\textbf{Relation Linking}} & \multicolumn{3}{c}{\textbf{Entity Linking}} & \\
        \textbf{System}&{\textbf{Precision}} &{\textbf{Recall}} &{\textbf{Macro F1}} &{\textbf{Precision}} &{\textbf{Recall}} &{\textbf{Macro F1}} & \textbf{QA F1 score}\\
        \hline 
        gAnswer   	& 8.05 & 8.18 & 7.76 & 19.74 & 20.00 & 19.54 & 8.18\\ 
        EDGQA   	& \textbf{59.44} & \textbf{53.95} & \textbf{56.56} & \textbf{73.85} & \textbf{68.75} & \textbf{71.18} & 53.1\\ 
        \textbf{{\sysName}} (ours)   & 7.29        & 41.03     &  10.95   & 59.95& 50.55 & 53.67 & 52.03\\ \hline 
        \end{tabular}
\end{table*}


==> tables/rpQuery.tex <==
\begin{table}[t]
% \ncp\ncp
\caption{$\mathcal{R_P}(g, v)$ query templates with different orientations.\shorten}
\label{tab:rpQuery}
\ncp\ncp\ncp\ncp
\begin{tabular}{l|l}
\hline
Outgoing Query Template  & Incoming Query Template \\ \hline
   \textbf{Select} distinct ?$p_r$ ?$d_p$ &    \textbf{Select} distinct ?$p_r$ ?$d_p$ \\ 
   \textbf{Where} \{  & \textbf{Where} \{ \\
$v$ ?$p_r$ ?o . &   ?s ?$p_r$ $v$ .   \\
\textbf{Optional}\{?$p_r$ ?$p_a$ ?$d_p$.\} \} &  \textbf{Optional}\{?$p_r$ ?$p_a$ ?$d_p$.\}  \} \\ \hline
\end{tabular}
\ncp\ncp\ncp\ncp\ncp\ncp
\end{table}

==> tables/rvQuery.tex <==





%\begin{table}[h]
%\ncp\ncp
%\caption{A $\mathcal{R_V}(g, l_n)$ query template for different RDF engines.}
%\label{tab:rvQuery}
%\ncp\ncp\ncp\ncp
%\begin{tabular}{l|l}
%\hline
%\textit{Virtuoso} Query Template & \textit{Stardog} Query Template \\ \hline
%   \textbf{Select} distinct $?v$ ?$d_v$ &   \textbf{Select} distinct ?$v$ ?$d_v$ \\ 
%   \textbf{Where} \{ ?$v$ $p$ ?$d_v$ .  & \textbf{Where} \{ ?$v$ $p$ ?$d_v$ . \\
%?$d_v$ <bif:contains> $\mathcal{T}(l_n)$ . \} & ?$d_v$ <stardog:textMatch> $\mathcal{T}(l_n)$ . \}  \\
%\textbf{Limit} Max$_{VR}$ &  \textbf{Limit} Max$_{VR}$  \\ \hline
%\end{tabular}
%\ncp\ncp\ncp\ncp
%\end{table}

==> tables/setting.tex <==
\begin{table}[t] 
% \ncp\ncp
% h asks to places the floating element [h]ere.
  \caption{{KGQAn} System parameters}
%   \ncp\ncp\ncp
  \label{tab:settings}
    \begin{tabular}{lc}
        \hline
        \textbf{Parameter}&{\textbf{Value}} \\
        \hline
        % Number of Vertices & 1  \\
        Number of Edges & 20 \\
        Max number of answers & 40 \\
         Max Fetched Vertices & 400 \\
        % Max Fetched Edges & 300  \\ 
        \cline{1-2}\hline
    \end{tabular}
    % \ncp\ncp\ncp\ncp\ncp\ncp
\end{table}

==> tables/symbols.tex <==
\begin{table}[t] 
% \ncp\ncp
% h asks to places the floating element [h]ere.
  \caption{Symbols used in the system description}
%   \ncp\ncp\ncp
  \label{tab:dataset}
    \begin{tabular}{lc}
        \hline
        \textbf{Symbol}& \textbf{Description} \\
        \hline
        $q$ &  Input question  \\
        $q_i$ & Word i in question q \\
        T & List of Triple in question q \\
        $t_i$ & $i_{th}$ Triple in set T \\
        $answer_{dtype}$ & predicted answer data type \\
        $answer_{type}$ & predicted answer type \\
        P & Phrase Graph Pattern \\
        N & Nodes of P \\
        $n_i$ & node i in set N \\
        $l_i$ & label of node $n_i$ \\
        E & Edges of P \\
        $e_i$ & edge i in set E \\
        A & Annotated Phrase Graph Pattern \\
        $v_{candidates}$ & List of vertices matching $n_i$ \\
        $p_{candidates}$ & List of predicates matching $e_i$ \\
        $V_i$ & Vertices assigned to node $n_i$ \\
        $P_i$ & Predicates assigned to edge $e_i$ \\
        ans & answer list returned to the user \\
        $y$ & sequence representation of T \\
        $F$ & transformation function from T to y \\
        \hline
    \end{tabular}
% \ncp\ncp\ncp\ncp
\end{table}

%        MS Academic & 18 & \\

==> tables/taxonomyTables/taxoTrial.tex <==
\begin{table*}[t]% h asks to places the floating element [h]ere.
  \ncp\ncp
 \caption{The taxonomy of the benchmark questions depending on shapes of SPARQL query and the type of questions according to LC-QuAD 2.0~\cite{lcquad2}}
 \centering
\begin{tabular}{l|llll|llll|llll|llll|llll|lllll}

\cline{1-25}
\textbf{Query type}           & \multicolumn{4}{c|}{\textbf{Star}}                                                                                                                                    & \multicolumn{4}{c|}{\textbf{Path}}                                                                                                                                    & \multicolumn{4}{c|}{\textbf{Singe fact}}                                                                                                                              & \multicolumn{4}{c|}{\textbf{Fact with type}}                                                                                                                          & \multicolumn{4}{c|}{\textbf{Multi fact}}                                                                                                                              & \multicolumn{4}{c}{\textbf{Boolean}}                                                                                                                                  &   \\
\textbf{Benchmark}            & \begin{sideways}\# queries\end{sideways} & \begin{sideways}\textbf{KGQAn}\end{sideways} & \begin{sideways}EDGQA\end{sideways} & \begin{sideways}Ganswer\end{sideways} & \begin{sideways}\# queries\end{sideways} & \begin{sideways}\textbf{KGQAn}\end{sideways} & \begin{sideways}EDGQA\end{sideways} & \begin{sideways}Ganswer\end{sideways} & \begin{sideways}\# queries\end{sideways} & \begin{sideways}\textbf{KGQAn}\end{sideways} & \begin{sideways}EDGQA\end{sideways} & \begin{sideways}Ganswer\end{sideways} & \begin{sideways}\# queries\end{sideways} & \begin{sideways}\textbf{KGQAn}\end{sideways} & \begin{sideways}EDGQA\end{sideways} & \begin{sideways}Ganswer\end{sideways} & \begin{sideways}\# queries\end{sideways} & \begin{sideways}\textbf{KGQAn}\end{sideways} & \begin{sideways}EDGQA\end{sideways} & \begin{sideways}Ganswer\end{sideways} & \begin{sideways}\# queries\end{sideways} & \begin{sideways}\textbf{KGQAn}\end{sideways} & \begin{sideways}EDGQA\end{sideways} & \begin{sideways}Ganswer\end{sideways} &   \\ 
\cline{1-25}
QALD-9               & 131                                      & {\textbf{60}}                                  &   56                                  & 21                                      & 19                                       & 2                                   &      \textbf{5}                               & 0                                      & 81                                       & \textbf{46}                                 & 41                                    & 16                                      & 28                                       & 7                                   &  \textbf{8}                                   &   3                                    & 37                                       & 9                                   &     9                                &               2                        & 4                                        & 0                                   &        \textbf{3}                             &                 0                      &   \\
YAGO-B               & 92                                       & \textbf{63}                                  & 39                                  & 32                                    & 8                                        & \textbf{5}                                   & 4                                   & 3                                     & 87                                       &\textbf{61}                                 & 40                                  & 33                                    & 6                                        & \textbf{5}                                   &  3                                   &     2                                  & 6                                        & \textbf{2}                                   &      0                               &  0                                     & 1                                        & 0                                   &   0                                  &                                       0&   \\
DBLP-B               & 90                                       & \textbf{62}                                & 8                                     &           2                            & 10                                       & \textbf{6}                                   &             0                        &                        0               & 85                                       & \textbf{60}                                  &     8                                &  1                                     & 11                                       & \textbf{6}                                   &                            0         &                                    1  & 4                                        & \textbf{2}                                   & 0                                    &   0                                    & 0                                        & 0                                   &     0                                &                0                       &   \\
MAG-B                & 77                                       & \textbf{44}                                  & 4                                   & 0                                     & 23                                       & \textbf{9}                                   & 0                                   & 0                                     & 75                                       & \textbf{40}                                  &              4                       &                         0              & 7                                        & \textbf{2}                                   &             0                        &                        0               & 16                                       & \textbf{9}                                   & 0                                    &            0                           & 2                                        & \textbf{2}                                   & 0                                    &   0                                    &   \\ 
\cline{1-25}

\end{tabular}
\end{table*}



%  \ncp\ncp \ncp\ncp\ncp\ncp
%  \label{tab:maintaxonomy}
%         \begin{tabular}{lcc|cccc}
%         \hline
%         \multicolumn{1}{c}{\textbf{}}&  \multicolumn{2}{c}{\textbf{SPARQL}}&\multicolumn{4}{|c}{\textbf{Types of Questions}}\\
%         \textbf{Benchmarks}&\textbf{STAR} & \textbf{PATH} & {\textbf{Single Facts}} & {\textbf{Single Facts + Types}} &{\textbf{Multi Facts}} &{\textbf{Boolean}}\\
%         \hline
%         {\qald} & 131 & 19 & 81 & 28 & 37 & 04\\
%         YAGO-Bench & 92& 8 & 87 & 06 & 06 & 01 \\ 
%         DBLP-Bench & 90  & 10 & 85 & 11 & 04 & 0 \\ 
%         MAG-Bench &  77 & 23 & 75 & 07 & 16 & 02 
%         \\  \hline
        
% \end{tabular}
% \end{table*}




% \begin{table*}[t]


==> tables/taxonomyTables/taxonomyDBLP.tex <==
\begin{table*}[t]% h asks to places the floating element [h]ere.

 \caption{\#Questions solved/\#Total Questions for the given variety of questions in DBLP}
  \ncp\ncp \ncp\ncp\ncp\ncp
 \label{tab:dblptaxonomy}
        \begin{tabular}{lcc|cccc}
        \hline
        \multicolumn{1}{c}{\textbf{}}&  \multicolumn{2}{c}{\textbf{SPARQL}}&\multicolumn{4}{|c}{\textbf{Types of Questions}}\\
        \textbf{Systems}&\textbf{STAR} & \textbf{PATH} & {\textbf{Single Facts}} & {\textbf{Single Facts + Types}} &{\textbf{Multi Facts}} &{\textbf{Boolean}}\\
        \hline
        {\sysName} & 62/90
&6/10&
60/85&
6/11&
2/4&
0/0
\\
  EDGQA &8/90&
0/10&
8/85&
0/11&
0/4&
0/0
\\
GAnswer&2/90&
0/10&
1/85&
1/11&
0/4&
0/0    \\  \hline
        
\end{tabular}
\end{table*}


==> tables/taxonomyTables/taxonomyKGQAn.tex <==
\begin{table*}[h]%[t] h asks to places the floating element [h]ere.
%   \ncp\ncp
 \caption{\#Questions solved by {\sysName}/\#Total Questions in each category. {\sysName} outperforms in most of the types when compared to other systems: EDGQA and GAnswer}
  \ncp\ncp \ncp\ncp\ncp\ncp
 \label{tab:taxonomyonKgqan}
        \begin{tabular}{lcc|cccc}
        \hline
        \multicolumn{1}{c}{\textbf{}}&  \multicolumn{2}{c}{\textbf{SPARQL}}&\multicolumn{4}{|c}{\textbf{Types of Questions}}\\
        \textbf{Benchmarks}&\textbf{STAR} & \textbf{PATH} & {\textbf{Single Facts}} & {\textbf{Single Facts + Types}} &{\textbf{Multi Facts}} &{\textbf{Boolean}}\\
        \hline
        {\qald} & 60/131 & 02/19 & 46/81 & 07/28 & 09/37 & 0/4\\
        YAGO-Bench & 63/92 & 05/8 & 61/87 & 05/06 & 02/06 & 0/1 \\ 
        DBLP-Bench & 62/90  & 06/10 & 60/85 & 06/11 & 02/04 & 0/0 \\ 
        MAG-Bench &  44/77 & 09/23 & 40/75 & 02/07 & 09/16 & 2/2 
        \\  \hline
        
\end{tabular}
\end{table*}


==> tables/taxonomyTables/taxonomyMAG.tex <==
\begin{table*}[t]% h asks to places the floating element [h]ere.

 \caption{\#Questions solved/\#Total Questions for the given variety of questions in MAG}
  \ncp\ncp \ncp\ncp\ncp\ncp
 \label{tab:magtaxonomy}
        \begin{tabular}{lcc|cccc}
        \hline
        \multicolumn{1}{c}{\textbf{}}&  \multicolumn{2}{c}{\textbf{SPARQL}}&\multicolumn{4}{|c}{\textbf{Types of Questions}}\\
        \textbf{Systems}&\textbf{STAR} & \textbf{PATH} & {\textbf{Single Facts}} & {\textbf{Single Facts + Types}} &{\textbf{Multi Facts}} &{\textbf{Boolean}}\\
        \hline
        {\sysName} & 44/77
&09/23
&40/75
&02/7
&09/16
&2/2
\\
EDGQA & 4/77 &0/23&
04/75&
0/7&
0/16&
0/2\\
        GAnswer & 0/77
&0/23&
0/75&
0/7&
0/16&
0/2        \\  \hline
        
\end{tabular}
\end{table*}


==> tables/taxonomyTables/taxonomyQald9.tex <==
\begin{table*}[t]% h asks to places the floating element [h]ere.
 
 \caption{\#Questions solved/\#Total Questions for the given variety of questions in {\qald}}
  \ncp\ncp \ncp\ncp\ncp\ncp
 \label{tab:qald9taxonomy}
        \begin{tabular}{lcc|cccc}
        \hline
        \multicolumn{1}{c}{\textbf{}}&  \multicolumn{2}{c}{\textbf{SPARQL}}&\multicolumn{4}{|c}{\textbf{Types of Questions}}\\
        \textbf{Systems}&\textbf{STAR} & \textbf{PATH} & {\textbf{Single Facts}} & {\textbf{Single Facts + Types}} &{\textbf{Multi Facts}} &{\textbf{Boolean}}\\
        \hline
        {\sysName} & 60/131 & 2/19 & 46/81 & 7/28 & 9/37 & 0/4\\
        EDGQA & 56/131 & 5/19 & 41/81 & 8/28 & 9/37 & 3/4\\
        GAnswer & 21/131 & 0/19 & 16/81 & 3/28 & 2/37 & 0/4
        \\  \hline
        
\end{tabular}
\end{table*}


==> tables/taxonomyTables/taxonomyYAGO.tex <==
\begin{table*}[t]% h asks to places the floating element [h]ere.
  
 \caption{\#Questions solved/\#Total Questions for the given variety of questions in YAGO}
  \ncp\ncp \ncp\ncp\ncp\ncp
 \label{tab:yagotaxonomy}
        \begin{tabular}{lcc|cccc}
        \hline
        \multicolumn{1}{c}{\textbf{}}&  \multicolumn{2}{c}{\textbf{SPARQL}}&\multicolumn{4}{|c}{\textbf{Types of Questions}}\\
        \textbf{Systems}&\textbf{STAR} & \textbf{PATH} & {\textbf{Single Facts}} & {\textbf{Single Facts + Types}} &{\textbf{Multi Facts}} &{\textbf{Boolean}}\\
        \hline
        {\sysName} & 63/92
&5/8&
61/87&
5/6&
2/6&
0/1\\
EDGQA & 39/92
&4/8&
40/87&
3/6&
0/6&
0/1
\\
GAnswer &32/92&
3/8&
33/87&
2/6&
0/6&
0/1     \\  \hline
        
\end{tabular}
\end{table*}


==> tables/timePerTaskLcquad.tex <==
% \begin{table}[t]
%  \caption{Comparison between EDGQA and {\sysName} in terms of time taken to run each step of the pipeline on the LCQUAD-1.0}
%   \label{tab:perTaskTimelcquad}
%         \begin{tabular}{lccc}
%         \hline
%         \textbf{Systems}&{\textbf{Understanding}} &{\textbf{Linking}} &{\textbf{Execution}} \\
%         \hline
%         EDGQA&  1.9          &  6.6       &  3.1   \\ 
%         % EDGQA(No Cache)&            &         &     \\ 
%         KGQAn   &   6.5      & 0.23  & 0.15 \\ \cline{1-4}\hline 
%         \end{tabular}
% \end{table}

==> tables/timePerTaskQald.tex <==
% \begin{table}[t]
%  \caption{Comparison between EDGQA and {\sysName} in terms of time taken to run each step of the pipeline on the QALD9. All times in seconds}
%   \label{tab:perTaskTimeqald}
%         \begin{tabular}{lccc}
%         \hline
%         \textbf{Systems}&{\textbf{Understanding}} &{\textbf{Linking}} &{\textbf{Execution}} \\
%         \hline
%         EDGQA   	&      1.7      &    7.5     &  3.1   \\ \
%         KGQAn   &    4.7  & 0.35   & 0.22  \\ \cline{1-4}\hline 
%         \end{tabular}
% \end{table}

==> tables/v1_uris.tex <==
\begin{table}[t]% h asks to places the floating element [h]ere.
  \caption{Top-K URIs of vertices matching "Danish Straits", PREFIX  dbpedia: \url{http://dbpedia.org/resource/}}
  \label{tab:vertex1}
    \begin{tabular}{|c|c|}
    \hline
    \textbf{Vertex}&{\textbf{Score}} \\
    \hline
    dbpedia:Danish\_Straits & 0.602  \\
    \hline
    dbpedia:Danish\_straits & 0.602 \\
    \hline
    \end{tabular}
\end{table}

==> tables/v2_uri.tex <==
\begin{table}[t]% h asks to places the floating element [h]ere.
\caption{Top K URIs of vertices matching Kaliningrad", PREFIX  dbpedia: \url{http://dbpedia.org/resource/}}
\label{tab:vertex2}
    \begin{tabular}{|c|c|}
    \hline
    \textbf{Vertex}&{\textbf{Score}} \\
    \hline
    dbpedia:Kaliningrad & 1  \\
    \hline
    dbpedia:Yantar,\_Kaliningrad & 0.83  \\
    \hline
    \end{tabular}
\end{table}
